Exploring the Efficiency of Renewable Energy-based Modular Data Centers at Scale

Modular data centers (MDCs) that can be placed right at the energy farms and powered mostly by renewable energy, are proven to be a flexible and effective approach to lowering the carbon footprint of data centers. However, the main challenge of using renewable energy is the high variability of power produced, which implies large volatility in powering computing resources at MDCs, and degraded application performance due to the task evictions and migrations. This causes challenges for platform operators to decide the MDC deployment. To this end, we present SkyBox, a framework that employs a holistic and learning-based approach for platform operators to explore the efficient use of renewable energy with MDC deployment across geographical regions. SkyBox is driven by the insights based on our study of real-world power traces from a variety of renewable energy farms -- the predictable production of renewable energy and the complementary nature of energy production patterns across different renewable energy sources and locations. With these insights, SkyBox first uses the coefficient of variation metric to select the qualified renewable farms, and proposes a subgraph identification algorithm to identify a set of farms with complementary energy production patterns. After that, SkyBox enables smart workload placement and migrations to further tolerate the power variability. Our experiments with real power traces and datacenter workloads show that SkyBox has the lowest carbon emissions in comparison with current MDC deployment approaches. SkyBox also minimizes the impact of the power variability on cloud virtual machines, enabling rMDCs a practical solution of efficiently using renewable energy.

==> characterization.tex <==
\subsection{Workload and Applications}
% \subsection{Application characterizations}
\label{sec:eval:app-characterization}



% \shadi{@Jinghan: I would move this section to eval-> setup. Also, I would remvoe the first para and half of 2nd para and shrink the remaining. These details, seem like the workload characteristics used in eval. Not a fundamental design. In section 2, we have some characterization, there, you can add any missing design insights. and explain how migration overhead is computed in section 3.3. If these changes sound reasonable to you, I can make the changes.}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Categories of applications}
\footnotesize{
\begin{tabular}{|c|ccc|c|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{}} &
  \multicolumn{2}{c|}{One Time} &
  \multicolumn{1}{c|}{Persistent} &
  \multicolumn{1}{c|}{\multirow{2}{*}{Applications}} \\ \cline{2-4}
\multicolumn{1}{|c|}{} &
  \multicolumn{1}{c|}{Migration} &
  \multicolumn{1}{c|}{Recompute} &
  \multicolumn{1}{c|}{Network} &
  \multicolumn{1}{c|}{} \\ \hline
1 & High & High & High & --- \\  \hline
2 & Low  & High & High & --- \\ \hline
3 & High & Low  & High & MongoDB-Large   \\  \hline
4 & Low  & Low  & High & MongoDB \cite{mongodb} \\  \hline
5 & High & High & Low  & DNN-Large  \\  \hline
6 & Low  & High & Low  & --- \\  \hline
7 & High & Low  & Low  & DNN \cite{dnn}  \\  \hline
8 & Low  & Low  & Low  & Cofii-HPC \cite{cofii}  \\ \hline
\end{tabular}
}
\label{tab:app_categories}
\end{table}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=.45\textwidth]{figures/design/app_characterization.pdf}
%   \caption{Application characteristics}
%   \label{fig:design:app-characterization}
% \end{figure}

% \anup{Should we have a characterization section before design, like done in SlackSched?} \jinghan{We should keep this subsection. Also need to to introduce the three types of overhead somewhere before.}

% For our application scheduling formulation, we need a method for estimating various overheads an application may face due to running in our \siteName{} environment. Such a characterization allows us to make placement decisions that minimize these overheads and also maintain a mix of applications with different overheads so that \name{} has flexibility in choosing which applications to migrate when there are power mispredictions. 

% To facilitate the characterization, we first identify three types of overheads that application could incur due to the migration during the power fluctuation: (1) VM state migration; (2) loss of compute due to recomputation; and (3) latency overhead. We then categorize cloud applications based on these three overheads. 
In Table~\ref{tab:app_categories}, we identify eight categories of applications by selecting low or high ($>20\%$) for each type of overheads (as described in Section~\ref{sec:diverse-app-characteristics}). We exclude three types from discussion: (1) Apps in category one have high overheads in all the three types of overhead and hence they are not the target workloads for the VB setting; (2) Apps in category two and six have low state migration overhead but high recomputation overhead which reflects a poor design as they can reduce recomputation with more frequent checkpoints. For the other categories, we consider the following three  representative applications: seismic, DNN training, and database. We initialize each applications with all of its VMs in the same availability zone and emulate one migration by splitting its VMs across different zones. We characterize the incurred overheads in Figure~\ref{fig:design:app-characterization}.

\textbf{Cofii:} Cofii\cite{cofii} is a seismic imaging application built with the AzureClusterlessHPC framework. Its default setup includes 16 4-core VMs. As shown in Figure~\ref{fig:design:app-characterization}, the overhead mainly comes from VM migration. Cofii does not experience high latency overhead after migration as most of its compute can be handled locally and a global synchronization only happens at the end of each iteration. It also does not have high recomputation overhead after migration as it has a small time per iteration. Therefore, it is considered as category eight.

\textbf{DNN:} The DNN application\cite{dnn} built with the AzureClusterlessHPC runs VGG16 on a 20-core VM. In Figure~\ref{fig:design:app-characterization}, its has recomputation overhead due to the loss of compute from checkpoint and high state migration overhead. Therefore, it is considered as category seven. We scale the application by $5\times$ \jinghan{we can tune this to be larger} to create a new application DNN-Large in category five.

\textbf{DB:} We choose MongoDB\cite{mongodb} as the application in category four. In our application characterization with three MongoDB replicas and YCSB workloads, we observe $22\%$ latency overhead when the replicas are split into different availability zones (see Figure~\ref{fig:design:app-characterization}). Therefore, it is considered as category four. We scale the application by $5\times$ to create a new application DB-Large in category three.

\shadi{reduce descriptions above.}

\shadi{@jinghan: add 1-2 sentences on how we build the workload from this mix. e.g.,:
In the default setup, we use an equal mix (in term of number of cores) of the 5 different categories. For each category, we uniformly generate an application with average of X VMs (or something like this). We also perform a sensitivity analysis studying the impact of different ratios of category mixes. 
}

% From our characterization, we learned that there are various kinds of overheads an application might face, some might be one-time and others might be persistent. Further, different applications may incur these overheads to varying degrees. We classify applications into different categories based on degrees of different overheads. We describe our testbed and methodology for measuring various application overheads and classification in \S\ref{sec:eval}. \anup{We emulate \siteName{s} by instantiating virtual clusters in different regions/availability zones provided by Microsoft Azure. We try to match the geographic distances of the virtual clusters with those of \siteName sites. We measure VM allocation times, sizes of checkpoints or state, time to migrate the state and checkpoints, application slowdown when application is distributed across different virtual clusters.}

% We consider applications in machine learning, HPC and database domains. Specifically, we study (1) training of deep learning based image classifiers \anup{Is this correct?}, (2) a seismic imaging application~\cite{cofii}, and (3) a distributed transactional database~\cite{}. We break down overheads into two types: (1) one time overheads including VM allocation time, checkpoint or state migration, and re-computation after migration, (2) persistent overheads including added latency or reduced throughput when communicating VMs are allocated in different \siteName{} sites.

% \begin{figure}[tbp]
%     \centering
%     \includegraphics[width=.48\textwidth]{figures/overhead-types}
%     \caption{Various types of migration overheads and app categories.}
%     \label{fig:breakdown}
% \end{figure}

% Figure~\ref{fig:breakdown} shows where applications lie in terms of degree of their one-time and persistent overheads. \anup{Show table of mapping?} \anup{Is following correct?} Specifically, we find that the transnational database has high persistent overhead for synchronizing updates between replicas in different \siteName{s}, depending on the size of the database, the state migration overhead may be high or low, the re-computation overhead is relatively small. The deep learning application consists of highly parallel tasks in different VMs without much communication, with regular iterations which perform checkpoints, the size of these checkpoints is also small relative to the data being processed, as result these tend to have low onetime and persistent overheads. \anup{@Jinghan what about seismic, I am not sure exactly which one was profiled. I think they can lie in different category depending on the task being done.}

% \begin{figure}[tbp]
%     \centering
%     \includegraphics[width=.48\textwidth]{figures/breakdown.pdf}
%     \caption{Breakdown of application migration overheads. \textcolor{red}{New applications with checkpoints; higher overheads;}}
%     \label{fig:breakdown}
% \end{figure}

% Old
% \begin{itemize}
%     \item not all apps are equally migration friendly.
%     \item We identify two types of migration overheads: one time and persistent.
%     \item One-time overhead includes: VM allocation, Storage state migration, Re-computation
%     \item Persistent overhead includes: added latency or reduced throughput as a result of Network latency/bw. 
%     \item We classify datacenter applications into four categories (based on combinations of different levels of one-time overhead and persistent overhead)
%     \item provide some examples or a table of each category. 
%     \item As long as we have a healthy mix of easily migratable and non-migratable tasks, we can have an efficiently running DC across a subgraph. 
%     \item we have to leverage this mix when decide which/when to move an app
%     \item We profile the breakdown of overheads for different types of applications, including deep learning, HPC, and database. \shadi{should this be in eval?}
% \end{itemize}

==> discussion.tex <==
\section{Discussion}

\label{sec:discussion}


\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.46\textwidth}
        \centering
        \includegraphics[width=\textwidth,]{figures/evaluation/application_mix_a.pdf}
        \caption{Migration friendliness of application mix.}
        \label{fig:eval:variability:a}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.46\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={0 0.5cm 0 0}]{figures/evaluation/application_mix_b.pdf}
    
        \caption{Application distribution skew to each category.}
        \label{fig:eval:variability:b}
    \end{subfigure}
    \caption{Varying the workload distributions.}
    \vspace{1ex}
    \label{fig:eval:variability}
    \vspace{-5ex}
\end{figure}


\noindent
\textbf{\name{} vs. centralized renewable-based datacenters:}
An alternative approach for \siteName{} deployment is to deploy one centralized data center within each subgraph of complementary renewable sites. 
In such scenario, the \siteName{s} will transfer power across renewable farms via power transmission lines, instead of migrating application workloads 
through network cables. We argue that \name{} is more feasible for two reasons. First, the complementary renewable sites within a subgraph are 
usually far away from each other (hundreds of miles), and connecting them to one centralized \siteName{} introduces significantly 
high construction costs of power transmission lines ($500K$ -- $1.6M$ dollars per mile~\cite{josep:icdcs2014, transmission-cost-2, transmission-cost}).
However, network cables cost an order of magnitude less than the transmission lines 
($27K$ to $80K$ dollars per mile~\cite{fiber-nw-cost-1, fiber-nw-cost-2}).
%\siteName{s} can be connected to the the network already provisioned for current data centers to further reduce the cost.
Second, the subgraphs will change dynamically (see \mbox{$\S$\ref{sec:multi-VB}}). Statically connecting \siteName{s} to designated renewable 
farms will lose the flexibility, cause higher volatility in power generation, and introduce higher interference to applications 
(see the static subgraph selection in Figure~\mbox{\ref{fig:eval:dynamic-subgraph-identification}}).
 
\noindent
\textbf{Carbon emission cost:} We compare the carbon emission cost of \name{} to the non-renewable data centers. 
We use the HPE ProLiant DL360 Gen10 server \cite{hpe-server} as an example. The embodied carbon footprint of the server 
is $744.5$ kg CO$_2$e \cite{hpe-server, carbonexplorer:asplos2023}, and the per-core power consumption is $13.5$ Watt. 
In our evaluation, \name{} deploys $923$ 16-core servers in total, and it powers 6,301 cores on average. 
As \name{} fully utilizes renewable energy, and the operational carbon emission of renewable energy ($11\sim41$ gCO$_2$eq/kWh) 
is significantly smaller than the non-renewable energy ($490\sim820$ gCO$_2$eq/kWh)~\cite{carbonexplorer:asplos2023}, 
\name{} can save $447.75$ tons of CO$_2$e per year (or $4.5K$ tons for a ten-year server lifetime) 
from the operation carbon emission, in comparison with the non-renewable data center. 
Even though \name{} requires more servers to provide the same computing resources due to the power variability, 
the additional embodied emission cost is $393.93$ tons of CO$_2$e, but this cost only happens once over the entire lifetime. Therefore, \name{} still has 
significantly less carbon emission, compared to a non-renewable data center. 

% \myparagraph{How \name{} Works with the Traditional Cloud}
% \hl{\mbox{\name{}} does not aim to replace the traditional data center design. Instead, we believe that \mbox{\name{}} complement with the existing cloud platforms.
% }
% josep:icdcs2014,



==> obsolete.tex <==
\newpage
\section{Obsolete}

 \begin{figure}[t]
  \centering
  \includegraphics[width=.4\textwidth]{./figures/design/migr_profile.png}
	 \vspace{-2ex}
	 \caption{Migration profiling }
  \label{fig:design:migr-profile}
	 \vspace{-2ex}
\end{figure}

\subsection{Characterization of VM Migration}
\label{sec:vm-charaterization}
% transition from the subgraph identification: live migration is needed, what is the commonly used migration methods what migration greenbox is using and what 
% to better understand the migration overhead, what experiments setup we are using
% the characteristic experiements and insights got from the experiments
% based on the insights, what assumption and setup we assume (network throttling)
\hl{
Subgraph identification can help achieve a stable aggregated power supply within each subgraph, but each individual \mbox{\siteName{}} still suffers from the power variability. 
To take advantage of the aggregated power in subgraphs, we utilize VM migration to transfer VMs from a site with transient power shortage to another site with sufficient power supply. 
However, VM migration is not a free lunch, but it introduces overheads to both the source server and the destination server due to additional computing and network resources required during the migration.
To minimize the overhead, \mbox{\name{}} employs the pre-copy live migration mechanism.
Compared with the other migration techniques (e.g. non-live migration or post-copy live migration), pre-copy live migration can minimize the amount of downtime and effectively tolerate network failures \mbox{\cite{}}. 
}

\hl{
Even with pre-copy live migration, unavoidable migration overhead comes from extra power consumption on both source server and destination server. 
To better understand the overhead, we build a platform based on Openstack \mbox{\cite{}}, and measure the additional power consumption brought by VM live migration using xxx meter with various VM sizes and network bandwidth. In our setup, we assume VMs run with 30\% CPU utilization on average and each VM migration should complete before its deadline.
}

\hl{
As Figure \mbox{\ref{fig:design:migr-profile}} shows, memory size of the migrated VM is linearly correlated with the total migration energy cost. This is because with a fixed network bandwidth, the migration time increases proportionally with the increase of the memory size, while extra power usage keeps static. Typically, in our setup, a VM with 16GB memory takes 160 secs to complete migration, and the extra power draw is 30 watts with an idle power of 177 watts.
}

\hl{
On the other hand, the network bandwidth is linearly correlated with the migration time, and higher network bandwidth leads to greater extra power consumption (see Figure \mbox{\ref{fig:design:migr-profile}}). 
However, the total migration energy is stable regardless of the network bandwidth. This insight motivates us to throttle network bandwidth flexibly to achieve lower power consumption without missing the deadline of VM migration.
The characteristic results of live migration is validated with several prior work\mbox{\cite{}}. 
Based on the observations, we build power models for live migration and these are incorporated into our optimization model.
}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{./figures/design/design_tradeoff.pdf}
%     \caption{Design considerations of application placement and migration of \name{}}
%     \label{fig:design_tradeoff}
% \end{figure*}



\subsection{5.2}
As discussed in \S\ref{subsec:site-identification}, \name{} supports two different site pruning policies: (1) \texttt{stable}, which selects the site with the highest minimum power production over a seven-day window, and (2) \texttt{cov-aware}, which selects sites with the lowest coefficient of variation over a seven-day window. \name{} uses \texttt{cov-aware} as the default policy, as it can identify sites that have less power variations. We show this by comparing \name{} with a baseline site pruning policy which randomly prunes \siteName{s}. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.47\textwidth,trim={0 0.6cm 0 0}]{figures/evaluation/power_traces.pdf}
%     \vspace{-1ex}
%     \caption{Power variability of the selected sites with different site pruning policies.}
%     \label{fig:eval:total-power-site-selection}
%     \vspace{-3ex}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=.45\textwidth]{figures/evaluation/site_identification_perf_summary.pdf}
    \caption{Comparison of different site pruning policies.}
    \label{fig:eval:site-identification}
    \vspace{-4ex}
\end{figure}


As shown in Figure~\ref{fig:eval:total-power-site-selection}, we demonstrate that the \texttt{cov-aware} policy smoothens the power production curve. Specifically, compared to the random policy, \texttt{cov-aware} policy lowers the coefficient-of-variance from $0.38$ to $0.22$.
% 
% \name{} can reduce the average coefficient of variation (CoV) of the power production per site from $0.39$ to $0.22$ with the best site identification policy. The power production curve are smoothened with the best site identification policy. \anup{Reframe as ``XYZ is best site identification and hence, we use that for \name.'' Or in the beginning, say, ``\name{} uses CoV policy, we compare this against two other policies: random and stable.''}

% We vary the site pruning policy while using the baseline policy for other steps (subgraph identification, application placement). We focus on two metrics: (1) the variability of aggregated power production and (2) the impact on the application performance.

We also measure the impact of site pruning policies on the performance of applications, as shown in Figure~\ref{fig:eval:site-identification}. The average slowdown of the applications is reduced from $1.27\times$ to $1.18\times$, and the 95th percentile slowdown of the applications is significantly reduced from $3.0\times$ to $1.71\times$. This is because the \texttt{cov-aware} site pruning policy identifies \siteName{s} with the least variation, which helps minimize the interruptions on applications. For applications affected by migration and blackout, we reduced the slowdown from $2.3\times$ to $1.73\times$.

\subsection{5.3 Impact of Subgraph Identification}
\label{sec:eval:subgraph-identification}
\zibo{this section should be incorporated into the previous section}

% In this section, we compare different subgraph identification policies: geolocation, stable, and CoV (coefficient of variation). 
With the optimized site candidates selected by the \texttt{cov-aware} site pruning, we now evaluate the effectiveness of subgraph identification by comparing three different policies:
(1) \texttt{geolocation}, which minimizes the average distances between sites, (2) \texttt{stable}, which maximizes the minimum aggregated power produced of the sites over a window of time (seven days in our setup), and (3) \texttt{cov-aware}, which minimizes the coefficient of variation of power samples from the aggregate power produced by the sites. 


% \jinghan{Make sure we keep the number of apps the same so that the baseline of this step matches with the optimal solution of the last step}
% \maybe{Frame as power-aware vs non-power-aware metrics. Power-aware policies are better.}
Figure~\ref{fig:eval:overhead-subgraph-identification} shows that both power-aware policies, \texttt{stable} and \texttt{cov-aware}, have significant improvement over the non-power-aware policy. The average slowdown of the applications is reduced from $1.18\times$ to $1.12\times$ (with \texttt{stable} policy) and the 95th percentile slowdown of the applications is reduced from $1.71\times$ to $1.50\times$ (with  \texttt{cov-aware} policy). For the affected applications, their slowdown is reduced from $1.74\times$ to $1.48\times$ (with \texttt{stable} policy). Therefore, we use \texttt{stable} as our default policy as it provides the best overall performance.

We also evaluate the subgraph re-identification (\S\ref{subsec:subgraph-identification}) of \name{} over a seven-week period. 
%study dynamic reselection over a seven-week period (\S\ref{subsec:subgraph-identification}). 
With dynamic subgraph identification, \name{} re-identifies the stablest subgraphs on a per-week basis, and helps increase the average stable power by $41\%$, as shown in Figure~\ref{eval:dynamic-subgraph-identification:a}.
Since we have more stable power to supply applications, the 95th percentile slowdown of applications decreases from $1.68\times$ to $1.50\times$, as shown in Figure~\ref{eval:dynamic-subgraph-identification:b}. Although the dynamic subgraph identification may cause application migrations (due to the subgraph update), 
its benefits on the application performance outweigh its overheads. This is because the dynamic subgraph identification will bring less-variable power to \siteName{s}. 
%This indicates that the benefits of less-variable power outweigh the inter-subgraph migration overhead, 
%because of the dynamic subgraph re-identification.
% . We also observe an overall benefit as the reduced the overall slowdown from $1.68\times$ to $1.50\times$ due to increase stable power outweighs the inter-subgraph migration overhead due to dynamic reselection.
% \shadi{isn't the conclusion of fig 11, that we should use stable?}


\begin{figure}[t]
    \centering
    \includegraphics[width=.45\textwidth]{figures/evaluation/site_selection_stable_perf_summary.pdf}
    \vspace{-1ex}
    \caption{Comparison of application placement policies.}
    \label{fig:eval:overhead-site-selection}
    \vspace{-2.5ex}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=.45\textwidth]{figures/evaluation/migrated_cores.pdf}
    \vspace{-1ex}
    \caption{Aggregated migrated cores for different policies.}
    \label{fig:eval:agg_migrated_cores}
    \vspace{-3ex}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.45\textwidth]{figures/evaluation/overhead_breakdown.pdf}
%     \caption{Breakdown of different types of overheads.
%     % \jinghan{show the percentage relative to lifetime of apps} \anup{What is black region in MIP?}\jinghan{they are still colored bars but just too thin}
%     }
%     \label{fig:eval:latency-breakdown}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=.45\textwidth,trim={0 0.6cm 0 0.3cm}]{figures/evaluation/affected_breakdown.pdf}
    \caption{Breakdown of the affected applications.}
    \label{fig:eval:app-breakdown}
    \vspace{-2ex}
\end{figure}

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/evaluation/misprediction_a.pdf}
        \caption{Power production}
        \label{fig:eval:misprediction:a}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/evaluation/misprediction_b.pdf}
        \caption{Application execution time}
        \label{fig:eval:misprediction:b}
    \end{subfigure}
    \caption{Robustness to mispredictions.}
    \label{fig:eval:misprediction}
    \vspace{-4ex}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.4\textwidth]{figures/evaluation/agg_migration_overhead.png}
%     \caption{Aggregated migrated overheads for different policies.}
%     \label{fig:eval:agg_migrated_overheads}
% \end{figure}

\subsection{5.4 vm placement and migration}
Based on the optimized set of subgraphs identified by subgraph identification, we now evaluate application placement by comparing four different policies: (1) \texttt{greedy}, which always allocates applications with the largest resource requirements to the sites with the most abundant power supply, and always migrates applications with the largest resource requirements; (2) \texttt{greedy-fair}, which is similar to greedy policy, but provides additional fairness by always migrating equal amount of VMs per application; (3) \texttt{MIP}, which uses the MIP model discussed in (\S\ref{sec:app-placement} and \S\ref{sec:app-migration}) for application placement and migrate; and (4) \texttt{MIP-app}, which uses the same MIP model but without future power predictions. 
% The greedy policy is only aware of per-site instantaneous power production and per-application power requirements. The greedy-fair policy additionally provides fairness by migrating an equal number of VMs per application at any migration point.
% The MIP-app policy, in addition, is aware of application characteristics (migration overheads, execution times), while the MIP policy, in addition, is aware of per-site future power predictions. 

% Greedy policy is neither aware of the application characteristics nor the power prediction. It greedily fills the VMs at each \siteName{} site as many as possible. Greedy-fair policy additionally migrates equals number of VMs per each application to ensure fairness. \anup{Unclear, maybe remove greedy-fair if it doesn't add any value.} MIP policy optimizes the MIP model described in $\S$\ref{subsection:scheduling}, which is aware of both application characteristics and the power prediction. MIP-app policy has the application knowledge, but it does not look ahead for the future power prediction.

We compare different application placement and migration policies in Figure~\ref{fig:eval:overhead-site-selection}. The average slowdown of applications is already significantly reduced by $1.12\times$ with the first two core components: site pruning and subgraph identification. With MIP as the application placement policy, the average slowdown is further reduced by $1.03\times$. MIP also reduces the 95 percentile slowdown of the applications from $1.60\times$ to $1.12\times$.
MIP and MIP-app both reduce the slowdown of affected applications (reduction from $1.48 \times$ to $1.24-1.32\times$), since both of them are aware of the application characteristics, and have a higher priority to migrate the migration-insensitive applications. In addition, since MIP is aware of the power prediction, it reduces the number of VMs that need to be migrated. Since each VM may have different number of cores (as its computing resource), we use the total number of cores of these VMs to quantify the migration overhead. As shown in Figure~\ref{fig:eval:agg_migrated_cores}, it reduces the total number of migrated cores by $2.98\times$ by placing long applications on \siteName{s} with sustained power, and shorter ones on \siteName{s} that are more volatile. The MIP scheme also reduces the percentage of affected applications from $28.4\%$ to $10.4\%$.

% Figure~\ref{fig:eval:latency-breakdown} shows the breakdown of application slowdown in terms of different overheads. MIP eliminates allocation $+$ recomputation $+$ latency overheads of the applications. The remaining overhead in MIP is due to blackout, which happens when there are no candidate \siteName{s} to move an application to in presence of a power drop, and queuing, which happens when there are no good \siteName{s} to place an incoming application. While MIP reduces these overheads by better planning into the future, they are also dependent on application arrival, resource requirements, and power production which cannot be fully avoided. On aggregate, the MIP policy reduces overheads by $8.8\times$ compared to Greedy. 



To further understand the impact of the placement and migration policies on different applications, we 
show the percentages of affected applications under each policy in Figure~\ref{fig:eval:app-breakdown}. 
%Figure~\ref{fig:eval:app-breakdown} shows the percentage of affected applications in each category. 
MIP achieves better scheduling efficiency by avoiding the migration of migration-sensitive applications (DL-Large and DB-Large). In comparison to Greedy, the number of affected Cofii applications (migration-insensitive) is reduced by $31\%$, while the number of affected DL-Large and DB-Large (migration-sensitive) is reduced by $58\%$ and $72\%$, respectively.


In summary, we observe that the application placement and migration of \mbox{\name{}} improve application performance for three reasons. First, \mbox{\name{}} schedules migration-sensitive applications to \siteName{s} that have more stable power production. Second, it places short-lived applications to \siteName{s} with shorter predicted resource availability, and applications with long execution time to \siteName{s} that expected to retain stable power for a longer time. Third, \mbox{\name{}} always prefers to move migration-insensitive applications. 



\subsection{5.5 Robustness and Sensitivity Analysis}

\noindent
%\textbf{Mispredictions in power production and application execution time:}
\textbf{Mispredictions.}
To study the robustness of \name{} against the prediction of power production, 
and the execution time of applications, 
we inject uniform mispredictions into the MIP model. 
We use the experiment setting as described in \S\ref{sec:eval:scheduling}.
Consider that the mean misprediction rate of one-day-ahead power prediction is less than $30\%$ (\S\ref{sec:predictability}), 
we vary the maximum misprediction ratio of the power production from $-60\%$ (underpredict) to $60\%$ (overpredict), and evaluate the application performance. In Figure~\ref{fig:eval:misprediction:a}, we show that the 95th percentile slowdown under power misprediction increases from $1.09\times$ to $1.17\times$, and the percentage of affected applications increases from  $10.4\%$ to $15.7\%$. 

In Figure~\ref{fig:eval:misprediction:b}, we vary the misprediction ratio of application execution time using the same methodology as discussed above. The 95th percentile slowdown under power misprediction increases from $1.09\times$ to $1.17\times$, and the percentage of affected applications increases from  $10.4\%$ to $11.8\%$. We observe that the overprediction of the execution time behaves worse than the underprediction in general. This is because short-lived applications are placed in a limited number of stable \siteName{s}, due to the overprediction of their execution time, while actual long-lived applications are placed in \siteName{s} with high power variance. This means that more long-lived applications need to be migrated when power variation occurs. However, \name{} still outperform the baseline policies. 
%which have at least $1.32\times$ for the 95th percentile slowdown and $24.0\%$ of affected applications.
\zibo{remove misprediction section here}
 
\begin{figure}[t]
  \centering
  \includegraphics[width=.4\textwidth]{./figures/evaluation/vm_distr.png}
	 \vspace{-2ex}
	 \caption{Sensitivity analysis of VM distribution and migration overhead}
  \label{fig:eval:sensitivity}
	 \vspace{-2ex}
\end{figure}

==> tex/hotnets/abstract.tex <==

\begin{abstract}
Renewable energy is becoming an important power source for data centers, especially with the zero-carbon waste pledges made by big cloud providers. However, one of the main challenges of renewable energy sources is the high variability of power produced.
Traditional approaches such as batteries or transmitting to the grid fall short on scale, overhead, or "green-ness". We propose Virtual Battery: instead of adapting the availability of power to match the computation demand we shift computational demand to meet the availability of power.
Virtual batteries shift demand by requiring applications to either be flexible and delay-tolerant or proactively migrating to where power is (going to be) available. We show that using multiple virtual battery sites in combination can meet the needs of modern applications. Moreover, we show how an intelligent network and power aware co-scheduler can not only provide availability despite variability but also help mitigate migration related network overhead by over 30\% in total and 4.2$\times$ at peak.
\end{abstract}

==> tex/hotnets/availability.tex <==
\section{Virtual Battery}
In this section, we analyze the feasibility of a Virtual Battery (VB) by answering three main questions: (1) Do VBs make sense from an economic standpoint? (2) How variable are renewable sources? (3) Can we absorb this variability while maintaining availability for VMs? 


\subsection{Economic Motivation}
\label{sec:VB-design}
VBs place data-centers \textit{right alongside the} energy farms creating a distributed cluster of edge data-centers (Figure~\ref{fig:arch}). This design brings-up a main question: \textbf{\textit{Why does VB make economic sense?}}
% \anup{Can remove this para. the para after the section heading introduces this.}

% \anup{We see four main reasons for \textbf{``why VB makes economic sense''.}}
We see four main reasons. First, VBs will be powered (almost) entirely by renewable energy, rather than an opaque source when using the grid, an important goal for cloud providers~\cite{azurepledge,pledge,googlepledge}. Second, the total datacenter cost can be reduced by $\approx$10\% (= 20\% * 50\%). 20\% of data center operating cost is due to power~\cite{powercost}, and 50\% of power expense is due to transmission~\cite{powercost}. Co-locating data centers obviates this transmission expense.
% } Power cost of a data center is around 20\% of its operating costs~\cite{powercost} and co-locating data centers with renewable sources avoids $\approx$50\% cost overhead of transmission and distribution of energy. 
Third, the growing penetration of renewables has increasingly caused grid operators to \textit{force} renewable farms to \textit{reduce} their output to maintain supply-demand balance~\cite{o2020too}. This is done by either i. capping the renewable generation (as high as  6\% of the overall renewable generation and increasing each year~\cite{indiacurtail,germanycurtail}) or ii. dropping the marginal wholesale price of power to very low levels including negative prices~\cite{negativeprices}, a phenomenon exacerbating with increased renewable penetration~\cite{kyritsis2017electricity}. VBs can not only use this energy, but also generate high value from it. 
% 
% This reduction is as high as 6\% of the overall renewable generation in a few countries and is showing an increasing trend each year~\cite{indiacurtail,germanycurtail}. VBs can flexibly absorb this extra power. 
% Fourth, even when power is not capped, the marginal wholesale price of power in energy markets can drop to very low levels including negative prices~\cite{negativeprices}, which is a phenomenon exacerbating with the current trend of increased renewable penetration~\cite{kyritsis2017electricity}. VBs can not only use this energy, but also generate high value from it. 
% 
Finally, bringing edge data-centers to any remote location has become increasingly simpler and more common, e.g., with  modular data centers that are connected anywhere~\cite{mdc}.
% using high-speed low earth orbit (LEO) satellite connectivity~\cite{azure-space}. 

% And this phenomenon of low and negative wholesale prices will increase with increased renewable penetration. Indeed, flexibility resources like Virtual batteries will be {\it paid} to flex up and flex down to absorb this excess volatility. The combination of lower average energy prices, and being paid to provide flexibility and absorb volatility lowers unit economics of both the flexible compute and the unit economics of providing flexibility and absorbing renewables' volatility. Finally, bringing edge data-centers to any remote location has become increasingly simpler and more common, e.g., with  modular data centers~\cite{mdc}, and affordable connectivity via low earth orbit (LEO) satellite high-speed, low latency networks.} \shadi{@Srini/Shiv, can you read and edit?}



% \srini{\textbf{Economic rationale for Virtual Battery:} The power cost for a data center is around 20\% of its operating costs~\cite{powercost}. In the virtual battery setup, co-location of data centers with renewable sources avoids transmission and distribution overheads ($\approx$50\%), leading to lower landed cost of electricity and subsequent increase in operational cost savings. Moreover, through \textit{modular data centers}~\cite{mdc}, cloud operators can bring data centers closer to the edge with satellite-based connectivity.  Virtual batteries will also help renewable farm owners. The growing penetration of renewables has increasingly forced grid operators to curtail excess power to maintain supply-demand balance~\cite{o2020too}. The curtailed power is as high as 6\% of the overall renewable generation in a few countries and is showing an increasing trend each year~\cite{indiacurtail,germanycurtail}. With an onsite virtual battery with the flexibility to absorb excess power, renewable operators can increase their revenue by selling energy to cloud operators. Thus, virtual batteries offer a win-win for both cloud operators and renewable farm owners.}
% % . we are changing the scale. modular dc, movign compute to edge datacenters. AFO. }

% By doing so, computation becomes more geographically distributed and closer to the end user \anup{Is power farm owner the end user?}, e.g., there are $>$42,000  utility-scale wind~\cite{windfarm} and solar~\cite{solarfarm} farms in the world, whereas, only 541 hyperscale data centers~\cite{eureport}. 

%Virtual Battery eliminates the 40-60\% overhead of transmitting and distributed power to a central location. However, it introduces the challenge of handling variable computation capacity.


% and 3. What are the related overheads of reducing variability (Section~\ref{sec:nw-overhead})? \anirudh{4. Can we support large scale applications?}


% 
% \begin{figure*}[]
% \centering
% \begin{subfigure}{.32\linewidth}
%   \centering
%   \includegraphics[width=0.9\linewidth]{figures/solar-WestFlanders.png}  
%   \caption{solar}
%   \label{fig:solar-variability}
% \end{subfigure}
% \begin{subfigure}{.32\linewidth}
%   \centering
%   \includegraphics[width=0.9\linewidth]{figures/wind-4days.png}  
%   \caption{wind}
%   \label{fig:wind-variability}
% \end{subfigure}
% \begin{subfigure}{.32\linewidth}
%   \centering
%   \includegraphics[width=0.9\linewidth]{figures/variability-cdf.png}  
%   \caption{wind}
%   \label{fig:variability-cdf}
% \end{subfigure}
% \caption{Variability in energy production, normalized by the max capacity, for two different resources (a) solar and (b) wind alongside (c) the CDF of power generation across a \shadi{X}month trace }
% \label{fig:variability}
% \end{figure*}

\begin{figure}[]
\centering
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\textwidth]{figures/renewable_data_analysis/power_ts_colorized.pdf}
  \vspace{-2em}
  \caption{Power variation over time}
  \label{fig:solar-variability}
  \label{fig:wind-variability}
\end{subfigure}
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\textwidth]{figures/renewable_data_analysis/Antwerp_CDF.pdf}  
  \vspace{-2em}
  \caption{CDF of power generation over a year}
  \label{fig:variability-cdf}
\end{subfigure}
% \vspace{-1em}
\caption{\small Quantifying Variability for solar and wind. %\shadi{@anup/srini: can you make the colors match for a) i.e., make solar blue}
}  
% \vspace{-1.5em}
%Variability in energy production, normalized by the max capacity, for two different resources (a) solar and (b) wind alongside (c) the CDF of power generation across a \shadi{X}month trace 
\label{fig:variability}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Variability of Renewables}
\label{sec:variability}
 
Renewables are volatile energy sources--their production depends on several external and uncontrollable factors. We quantify the variability of two main energy sources, solar and wind, by analyzing two datasets: the EMHIRES dataset~\cite{iratxe2016emhires, gonzalez2017emhires} with traces from $>$500 sites in Europe, and the ELIA dataset~\cite{elia}, a fine-granularity dataset (15 min) from 25 sites in Belgium which also includes per-site energy forecasts.
% Along with the generation data, ELIA dataset also contains week-ahead, day-ahead, and 3hour-ahead forecasts.
%\shadi{name of dataset +cite} 
%energy traces.
% , therefore, creating both short and long term variability. 

We see large amount of variability across space (different locations), time (times of the day, seasons, etc.), and different resources (solar, wind, etc).
Figure~\ref{fig:solar-variability} shows a 4 day sample of solar production (ELIA dataset), normalized to the max production capacity. As shown, solar energy follows a periodic diurnal pattern, but days overcast with heavy clouds can significantly reduce the peak production (3.5\% vs 77\% the following day), and days with variable cloud patterns cause spiky energy production. Change of seasons similarly cause variability, e.g., peak production in winter is $\approx$75\% less than summer. 
% Location also has significant impact as two neighboring regions can have completely different weather conditions.
% , e.g., in the same Europe region, Portugal has on average 307 sunny days a year, while Belgium has only 132.
Different energy sources exhibit different patterns. As shown in Figure~\ref{fig:wind-variability}, wind energy production for the same duration exhibits sharp peaks and valleys (depending on weather conditions), but rarely go down to zero. %However, they also produce over 90\% of their maximum capacity only 1.2\% of the time periods.  

Figure~\ref{fig:variability-cdf}, shows the CDF of power generation over a year for wind and solar. 
Both sources exhibit large variability, with median values reaching at most 20\% the peak capacity for wind and over 50\% zero values for solar energy due to night times.
The tail is also high, with 99th divided by 75th percentile ratios of 4$\times$ for solar and 2$\times$ for wind.
% Similarly, the standard deviation was significantly high, 0.25 and 0.13 for solar and wind, respectively.


% We cluster the solar days into 3 categories: sunny (36\% of the days), overcast (17\% of the days), and variable (47\% of the days). \seshan{not sure why split into these 3 for this graph} 



% The tail production rarely reaches max capacity, e.g., 90^{th} percentile of wind, solar-sunny, solar-overcast are $< X, Y, and Z\%$ max production, respectively. 

%\shadi{@Srini-I, can you please fill in the numbers marked above?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Availability Despite Variability}
\label{sec:multi-VB}

\begin{figure}[]
    \centering
    \begin{subfigure}[t]{\columnwidth}
        \includegraphics[width=\textwidth]{figures/renewable_data_analysis/stacked_comb_purchased.pdf}
        \vspace{-2em}
        \caption{\textbf{Complementary power generation for 3 sites ---} When PT wind has higher production (green area), UK wind has lower production (orange area) (Day 4 to 5), and vice-versa. Shaded area denotes purchased energy (4000 MWhr).}
        \label{fig:multi-site}
    \end{subfigure}
    \begin{subfigure}[t]{\columnwidth}
        \includegraphics[width=\textwidth]{figures/comb_bar_stacked.pdf}
        \vspace{-2em}
        \caption{Break-down of stable \& variable energy.}
        \label{fig:sellable-vms}
    \end{subfigure}
    % \vspace{-1.5em}
    \caption{\small Reducing variability in energy production by aggregating multiple VB sites.}
    % \vspace{-1.5em}
\end{figure}

We target two class of applications. First, degradable applications that can adaptively be down-graded (similar to when using Harvest VM or Spot instances). 
Many scenarios can potentially use such degradable VMs such as batch or ML training jobs.  
% including long-running jobs with no hard deadlines, e.g., batch jobs, HPC workloads, ML trainging jobs; quickly transferable jobs with little state or no state, e.g., server-less computing, or coin mining; and opportunistic jobs, e.g., background compression of data.
The other category are stable VMs that require high levels of availability (similar to on-demand VMs in the cloud). This category provides higher value for the cloud providers and is the commonly used approach for most applications. Our goal is to maximize the number of stable VMs that this infrastructure can support. In this section, we explore a promising approach to reach this goal.


% However, many applications do not fall into these categories, and the ones that do are not usually developed in way to cope with degradable VMs.

% One option to cope with variability is to adaptively downgrade application resources, e.g., by - i) reducing the number of allocated resources such as in Harvest VMs~\cite{harvestvm}, Burstable VMs~\cite{azureburst,awsburst}, or Deflatable VMs~\cite{sharma2019resource}, ii) under-clocking the CPUs~\cite{oversubscript}, iii) preempting VMs such as in Spot instances~\cite{azurespot,awsspot}. We call such VMs ``degradable'' VMs. 
% Many scenarios can theoretically use such degradable VMs including long-running jobs with no hard deadlines, e.g., batch jobs, HPC workloads, ML trainging jobs; quickly transferable jobs with little state or no state, e.g., server-less functions \shadi{cite}, or coin mining; and opportunistic jobs, e.g., background compression of data. 
% However, many applications do not fall into these categories, and the ones that do are not usually developed in way to cope with degradable VMs. Also, for cloud providers, these options yield much less value than regular VMs, e.g. $\approx 90$\% discount in case of spot VMs~\cite{azurespotprice}. Thus, in an virtual battery environment, \textit{we would want to maximize the amount of normal (i.e., non-degradable) compute that we can run with cloud-level availability. } \seshan{reduce this paragraph -- this is just a transition motivation for 2.2. Just refer back to the intro text, "As mentioned earlier, our goal is to maximize the number of stable VMs that this infrastructure can support. To do this we must explore ways to xxx. We consider one such solution in the next section" }


Despite the large variability in a single renewable energy production site, we observed that these variability patterns are often independent and/or complimentary when looking at different sites or times of the day. This complimentary trend can be because of: a) using different energy sources (e.g., wind vs. solar at night time); b) effect of micro-climates or weather (e.g., same solar source but in two different locations, one of which is covered by clouds); or c) time of the day (e.g., day in one location and dusk in another).  

We leverage this insight and question, \textit{can we mask the variability in renewable energy sources by leveraging variability patterns across more than one site?}

We searched for complimentary groups of sites, all in close proximity of each other ($<$50ms ping latency), over 3 day intervals (in EMHIRES). Since our dataset only includes normalized power, we assume all sites have similar peak capacity of 400 MW--the median peak-capacity across large farms in the world~\cite{onshore-wind-wiki}\footnote{We could not find any public datasets with large number of sites spread geographically that have raw power values. We also note that the max power capacity ranges for both solar and wind are very similar~\cite{windfarm,solarfarm}}. We use the coefficient of variation, $cov$ (standard deviation divided by mean) as our comparison metric.
Based on our result, even when combining just two sites, $>52\%$ of possible 2-site combinations improved $cov$ by $>50\%$. 
% Similarly, for 3-site combinations, $>57\%$ of the combinations improved the the $cov$ by $>50\%$.
% \shadi{@Srini-I: add some stats here. For example, "Based on our results, for groups of size 2, 3, and 4 there was over 53\%, 81\%, and Z\% reduction in the average coefficient of variation by more than 30\%, respectively." You can use a different threshold, just not too low}  
% 
% 
Figure~\ref{fig:multi-site} demonstrates such an example as a stacked area graph, i.e., upper areas are added to all areas below them. As shown, the solar pattern in Norway (NO) when complemented with just one additional wind site (UK wind) reduces $cov$ by 3.7$\times$. Adding power from another wind source in Portugal (PT wind), further improves variability and reduces $cov$ by an additional 2.3$\times$. 

% \anirudh{break in flow here. name the para differently around the question rather than solution?}

% \noindent\textbf{Creating more normal (non-degradable) VMs:}
\smallskip\noindent\textbf{Does aggregation increase the stable capacity?}
We quantify the amount of \textit{stable} energy generated over a time window as: the minimum power level in the window multiplied by the size of a window. Since this energy is guaranteed to be available in that time window, it can reliably be used for stable VMs, and all remaining energy (called as variable energy) for degradable VMs (e.g., spot, harvest VMs).
As shown in Figure~\ref{fig:sellable-vms}, when we combine VB sites, larger portion of energy is stable, e.g., in ``NO+UK+PT'' 67\% of energy is stable while for ``NO+UK'' this value is 38\% stable. 

% \seshan{are there subtle points being made between the three para above? If not, perhaps a bit long for the info conveyed} \anup{I dont think there is anything subtle. Its just showing sites are uncorrelated and lead to lower power variability when aggregated.}

% Also, in this example, adding more sites to any combination of sites increases stable energy. For instance, ``NO+UK+PT'' has 18,000 MWhr stable energy while, ``NO+UK'' has 6,000 MWhr and ``PT'' has only 950 MWhr stable energy.

% Site StableEnergy TotalEnergy
% NO 0.0 2072.8920000000003
% UK 4892.064941176469 13987.272117647062
% PT 975.0714285714287 11102.003428571428
% NO + UK 6099.66014117647 16060.16411764706
% NO + PT 2203.9993142857147 13174.89542857143
% UK + PT 17116.702605042014 25089.275546218487
% NO + UK + PT 18165.638255462185 27162.16754621849


\smallskip\noindent\textbf{Would using a small reliable energy source alongside help?} Traditional ways, back-up generators, purchasing from the grid, and using batteries, all come with their individual trade-offs. However, using these techniques in small scales, just enough to cope with minor variability, can be a beneficial option economically. For example, we can try to fill in some of the worst gaps in the ``NO+UK+PT'' combination, shown as gray shaded areas in Figure~\ref{fig:multi-site}. In this case, by purchasing an additional 4,000 MWhr energy from the grid, we can stabilize 8,000 MWhr of variable energy and achieve a total additional 12,000 MWhr of stable energy. 


This multi-VB design introduces new networking challenges (\S\ref{sec:nw-overhead}) and power/economical challenges (\S\ref{sec:discussion}).

% \anup{For instance, we observe that if we purchase additional 10\% energy from the grid, we can convert 50\% of total renewable energy into stable energy.}
% \shadi{@Anup: show how buying a certain \% energy can improve the VMs sold.}



==> tex/hotnets/background.tex <==
\section{Background}

\shiv{Clearly state how we are different from other works}

\subsection{Grid Operations}
\shiv{Operators want to minimize imbalance, RE players want to maximize monetization.}

\subsection{Energy Markets}

\subsection{A case for micro Data Centers}

==> tex/hotnets/challenges.tex <==
\shadi{the following should probably each be a section or sub-section.}

\paragraph{\bf Challenges:}

\begin{itemize}
	\item \textbf{reliability:} amount of compute changes, how to ensure any SLAs? do we need new notions of SLA for this new env? do we need new programming paradigm for apps to degrade?
	\item \textbf{NW challenges} how to get the data required for compute to the VB site? NW challenges. what about when migrating?
	\item \textbf{economic benefits:} How to ensure this is greener, and has economic benefits (by leveraging fluctuations in the energy markets)? how much capacity to provision in each edge site? how to have an always full queue of workloads to run?
	\item \textbf{ incentivise users:} how to incetivize apps and users to use these green, but somewhat unreliable, resources?
	
\end{itemize}





\paragraph{\bf Solutions/ideas:}
\begin{itemize}
	\item \textbf{higher availability via multi-site VB:} one site has lots of variability and thus low reliability. Can we boost availability using multiple VB sites? 
	\newline [why would it work?] 1) different sites's energy sources can be independent (ex: one solar, one wind), 2) can have complimentary patterns (ex: solar and wind, sunny day vs cloudy+windy day), 3) patterns can be predicted in short-term time-scale
	\newline [how to leverage?] either a) replication: availability zones in independent sites or b) live migration.
	\newline [sub-idea: sun-synchronous geo-migration]. given predictable pattern of sun moving, move workloads following the sun pattern across solar farms.
	%%%%%%%%%%%%%%%
	\item \textbf{New abstractions: Green coin and green certificates.}
	%%%%%%%%%%%%%%%
	\item \textbf{picking NW aware \& migratable workloads} either a) don't need data, coin mining, b) data is much less than compute and can be prefetched, ML traning, read heavy DB c) data generated right there, satellite, IoT, drone, d) data generated and consumed there, 5G cell tower with AR workload.
	%%%%%%%%%%%%%%%
	\item \textbf{new programming paradigm: degradable apps}
	%%%%%%%%%%%%%%%
	\item \textbf{using deprected HW} economically cheaper.
\end{itemize}

==> tex/hotnets/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

==> tex/hotnets/cost.tex <==


\section{Economic Challenges}
\shadi{@Shiv \& Srini: can you help with this section and how you would like to structure it? I have put in a draft version.}

\srini{Compute markets and energy markets. Participation in multiple markets, value stacking and cross subsidies, multiple anticorrelated markets. }

By using the energy produces by renewable farms, right there in co-located mini data-centers, the cost of energy reduces by \shadi{2x?} by cutting all transfer cost. These include the overhead of selling to and then buying from the energy market, \shadi{@Shiv/Srini: please fill?}.  


However, running computation on virtual battery site introduces several new economic challenges.
First, higher availability is achieved by  higher resource usage (more replicas, migration cost, etc). We need to strike the right balance such that reaching higher availability does not make the cost of running a workload higher than the mainstream cloud prices. 
In addition, depending on the distributions of energy generation in a region, it might not be feasible to reach the same level of availability as the cloud at the same cost. In such cases, how can we incentivize applications and users to use these green, but somewhat less reliable, resources? 


Second, the energy market is a highly variable market. Figure \shadi{add graph} shows the pricing to sell/buy from the energy grid. At peak prices, it might make more economical sense to sell the energy instead of using it for compute. Also, energy can be stored and sold at later time when prices are high. Including these options (sell or store) as a potential destination of the energy, arbitrarily reduces the energy transferred to the compute cluster, thus, 
breaking the assumption that ``renewable energy can be predicted accurately''. \shadi{Is this point relevant to the paper? should we remove? }

Third, shutting down servers when energy production is low, reduces the utilization of the cluster--you have purchased and set-up hardware sitting powered-off in an edge datacenter. This brings up the question of capacity planning, i.e., how much hardware and what type of hardware should we provision, especially given that the energy could be sold to the energy market.

\srini{Highlight the approaches that can be implemented beyond shutting down and powering on servers. }

At the same time, there are several new research opportunities towards addressing these challenges:
\begin{itemize}
    \item \textbf{Using deprecated HW:} Cloud providers continually upgrade their mainstream hardware and sell the deprecated hardware for \shadi{10x?} cheaper than the original price. While such hardware might provide lower availability, the virtual battery environment is designed to handle high and sudden drops of capacity. An option would be to leverage these significantly cheaper hardware. 
    \item \textbf{Green certificates:} Companies are continually becoming more environmentally conscious. A systematic way to reward or incentives users to use an (almost) completely renewable-based compute is to introduce ``green certificates''.
    Similar to other industries, e.g., food with organic certificates, standardized compute certificates representing the level of \textit{greeness} can motivate users to embed reliability in their applications and leverage the green resources in virtual batteries.
    % \item \textbf{New markets--green coin:} coin mining is a great fit for variable resources. introduce a new concept, green coin, powered only by renewable. crypto-currency without harming the planet. challenges with how to cope with variability and not loosing progress
    \item \textbf{Smart scheduling of selling, storing, or using energy:} one potential option is to build models for the energy market pricing. While there are certain unpredictable factors in that market, there is also common patterns. These models can be used to smartly decide on when to store, sell, or use the energy for compute.
\end{itemize}



\subsection{Applications and Use-cases}

What type of applications can run in such a variable environment?
\begin{itemize}
	\item \textbf{preemptable \& no hard deadline:} can be paused, and resumed arbitrarily.
	ML training, batch jobs, hpc jobs? (not preemptable...).
	\item \textbf{Quickly Transferable:} either a) not much data associated, can be moved easily to another location, or b) data can be prefetched.
	\newline [example a)]	Small Azure Functions pushed to a renewable DC from the cloud. crypto mining.
	\newline [example b)] ML training over fixed dataset.
	\item \textbf{Degradable}: can be degraded based on compute available. 
	Can be latency sensitive.
	Example: having various ML models and adaptively using one.
	\item \textbf{Opportunistic:} not submitted by user, rather system predicting the need for it.
	Background compression of data that system predicts will be transferred
	\item \textbf{Hot replication:} latency sensitive apps can run (essentially can afford the extra compute const of replicated processing).
	\item \textbf{Data Generated onsite:} edge computing scenarios where data processed and result either uploaded to remote/cloud location or returned to user near the site, e.g., farms or commercial usecases uploading important information to cloud or sending alerts to technicians on site, 5G cell towers. 
\end{itemize}


==> tex/hotnets/discussion.tex <==
\section{Discussion and Conclusion}
\label{sec:discussion}

% \smallskip\noindent \textbf{Economic cost-benefit.} One concern with shutting down compute is the lost economic opportunity, where fully set-up hardware is not being utilized.
% One potential option is to use deprecated and refurbished hardware from bigger data centers for Virtual Batteries. While such hardware might provide lower availability, the virtual battery environment is designed for sudden drops of capacity. 

% % \anup{Cost of ownership is lower if servers are not powered right? cheaper electricity bill, no cooling cost at night for solar etc. If cost of ownership of server inside a VB site is infact lower, why is there an economic loss? Its a profit right, we sell at the same price (regular VM), but the cost is lower => larger relative profit than traditional DCs. At the same time lower carbon footprint...}


% % Virtual batteries involve a capital expense of the computation hardware and operations costs of remote monitoring/management of workloads. Monetization of virtual batteries happens by charging for compute and by charging for power usage flexibility. The unit economics of flexing power is lowered because computation also helps pay for the infrastructure. However, the periods of reduced power use mean that servers are shut down, and there is an opportunity cost of unused compute capacity. We are exploring both new and used (i.e., depreciated) compute hardware to optimize the overall unit economics of virtual batteries to be compelling to both the energy and compute ecosystems. Further, the opportunity cost of unused compute can be (partially) offset using lower energy costs due to avoidance of transmission and distribution overheads with co-location with renewables and substations. Moreover, the virtual battery can help renewable players to avoid curtailment from grid operators during periods of high power supply and low demand. 
% %Shutting down servers when energy production is low, reduces the utilization of the cluster--you have purchased and set-up hardware sitting powered-off in an edge datacenter. This brings up the question of capacity planning, i.e., how much hardware and what type of hardware should we provision, especially given that the energy could be sold to the energy market. \shadi{@Srini: rewrite.}

% % \noindent \textbf{Network-aware placement--picking the right mix of applications:} 
% % Not all applications create equal amount of migration/replication state. For example, a coin mining application has very limited state, a ML training application a can replicate the training data once and only migrate/replicate the models thereafter, while a database application would require continuous replication or large amount of data with low latency \shadi{better 3rd app?}. Maintaining a balance of applications with large and small amount of state in each location will enable the scheduler to move applications with small amount of state in majority of the cases and move the state-heavy application only when absolutely necessary. However, this should be done in fair way that also maintains the application requirements on availability, e.g., having certain number of replicas at all time. 


% \smallskip\noindent\textbf{A new programming paradigm---carbon-aware, degradable apps.} An alternative to just having two classes of application, background  vs. interactive, a third class of applications can choose how/when to degrade their computation.  Similar to  ``low power mode'' computation in battery-constrained environments such as mobile computing platforms, we envision a simple carbon-aware API exposed to applications which informs the applications when renewable power sources are running low alongside the carbon footprint of providing a given power level at that point of time. Then, applications can decide if and how to degrade.


\smallskip\noindent\textbf{Other challenges of multi-VB.}
Realizing the multi-VB design comes with a few additional challenges. First, the additional network overhead could require powering on network infrastructure that would otherwise be idle/off. However, we observe that migration occurs only 2-4\% of the time assuming 200Gbps WAN link per VB site (\S\ref{sec:nw-overhead}). Hence, the migration energy added by VB is negligible compared to upto 50\% energy loss in power transmission~\cite{power-loss}.
% } However, based on our results, the fraction of time spent in migration compared to normal execution (which represents the upper-bound of additional power overhead) is $<3\%$ which is negligible compared to 50\% loss in transmission (assuming 200Gbps WAN links).
Second, shutting down compute is the lost economic opportunity, where fully set-up hardware is not being utilized. This can be circumvented by using deprecated and refurbished hardware or purchasing power from the grid.
% } One option is 
% to use deprecated and refurbished hardware for a fraction of the cost. Also, the traditional way of relying on "purchasing from the grid" can be used in certain cases (Figure~\ref{fig:multi-site}). 
Finally, VB requires managing more number of (edge) data centers compared to a centralized design, thus, requiring additional one-time infrastructure (e.g., WAN connections, buildings, etc.) and maintenance. The community is already building edge data centers~\cite{zcc, freelunch}. VB adds to these efforts by providing high availability on-top.

\smallskip\noindent\textbf{Conclusion.} In this work, we investigate methods to build data centers with renewable energy. We propose Virtual Battery as an approach that adapts computation to accommodate power variations. In our approach, we envision data centers co-located with power generation to curb transmission costs. We observe that leveraging an ensemble of multiple sites significantly reduces variability at the cost of considerable network overhead. We finally propose a network and power-aware scheduler that reduces network overheads.

% For example, a stream processing app might prefer under-clocked workers but maintaining the same number of VMs/workers (to prevent moving state), while a ML training application might prefer to keep fewer high-capacity trainers (for faster convergence).  

% In addition, as users are becoming more environmentally cautious, the carbon footprint of running their application could become a important factor on if/when to degrade. If running the application when there is insufficient renewable energy comes at the cost of using non-renewable high-carbon resources, the user might decide to pause parts (or all) of the application and resume them in the future. 

% Similar to  ``low power mode'' computation in battery-constrained environments such as mobile computing platforms, we envision a simple carbon-aware API exposed to applications which informs the applications when renewable energy sources are running low alongside the carbon footprint of providing a given energy level at that point of time. Then, applications can decide if/how to degrade. Given the predictable nature of renewable resources, this API could also expose future options, e.g., carbon footprint will decrease by  50\% in the next 15 minute window. \shadi{shrink last part to one paragraph.}



==> tex/hotnets/intro-new.tex <==
\section{Introduction w/ Shiv's Edits}
\label{sec:intro}

% Climate change is the major challenge of our times. To avoid significant repercussions, we need to decarbonize our energy mix sources substantially. 

% Increasingly, governments~\cite{unsdg} and corporations~\cite{pledge} around the world have pledged to become ``carbon neutral'' or ``carbon negative'' in the near-term future. 
\shiv{cite}

%%%%::::: Renewable are the next big thing, but they are variable as well
Cloud computing has become a substantial source of carbon emission surpassing the aviation industry~\cite{lean-ict}. As a result, all major cloud providers have pledged to become ``carbon neutral or negative'' in the near-term future~\cite{pledge}. 
At the same time, the tremendous technological advancements in renewable energy sources has reduced their levelized cost of energy (LCOE) to values lower than traditional energy sources\shadi{cite}, making renewable energy a key to achieving carbon neutrality.  
% 
However, the biggest constraint for deep decarbonization, i.e. substantially higher penetration of renewable sources is how to absorb and manage the variation \& intermittency over time (volatility) in the renewable power produced that is not matched to demand. For example, solar produces no energy at night and daytime energy output varies with the presence of clouds and seasons of the year; and leads to a net demand increase in the evenings in high solar penetration regions (the "duck curve" in California \srini{cite}). Similarly, wind production ramps up and down  frequently throughout the day and seasons based on the direction and speed of wind. The conceptual solution to volatility is simple: either export it across \textit{space} (via transmission grids, larger imbalance regions (eg: Western imbalance region (WIB) in US, or interconnected European grid)), or \textit{time-shift} supply to meet demand (via energy storage or flexibility mechanisms); and managing this supply-demand mismatch at different time-scales via a variety of electricity markets (term-ahead, day-ahead, intra-day, real-time, ancillary markets). Since the cost and complexity of space-shifting excess energy is high, the fundamental constraint to deep decarbonization is lower-cost, flexibility resources in-situ at renewable energy plants \& inside the grid (eg: substations etc).  



% However, renewables, such as wind and solar, are intermittent sources of energy. Figure~\ref{fig:variability} shows variable energy generation from a few sample renewable sources. As shown, variability exists both in short (few minutes) and long (days or months) intervals. A wide range of factors ---such as seasonal changes, diurnal patterns, weather factors, cloud and wind movements --- cause such variability. 




%%%%%::::: Current solutions are not sufficient.
% When this variability results in such systems having excess energy, they store this energy for later use with grid-scale Li-Ion batteries, which come with  a limited life-cycle ($\approx 1000-3000$ discharge cycles \shadi{cite}), high carbon footprint for production\shadi{cite}, and loss of efficiency (\shadi{X\%} loss during charge \& discharge\shadi{cite}). To cope with energy shortfalls due to this variability, some systems either: i. rely on back-up generators from non-renewable sources with high carbon footprints, or ii. purchase energy from the ``energy market'' with dynamic (and often high) costs and unknown carbon footprints. 

% . A common practice is to store store energy during peak production for use at later times by using massive grid-scale Li-Ion batteries. However, physical batteries come with a limited number life-cycle ($\approx 1000-3000$ discharge cycles \seshan{do we have a citation for this}), high carbon footprint for production, and slow time-shifting between charge \& discharge (orders of \shadi{minutes?}) \seshan{any comment on efficiency losses?}. \shadi{citations, related works}. 
%We need an energy storage device which offers the ability to "time-shift" (charge/discharge) energy \textit{infinite} number of times and over \textit{different time scales} (milliseconds to months).



% In this work, we propose the concept of a \textit{``virtual battery'', i.e., using compute to emulate the fundamental behavior of an energy storage device--elastic time-shifting of energy (charge/discharge)--for infinite number of times.} 

%%%%%::: introduce problem statement and Virtual battery concept. 
In this work, we propose a paradigm shift:
\textit{Instead of bringing elastic power to computation, we can bring elastic cloud compute to the source of renewable power generation to absorb renewables volatility and drive deep decarbonization at scale}. The impact of absorbing renewables volatility is felt by the computation (via delayed execution and affecting availability). We propose to reconstruct a higher availability abstraction by leveraging virtual batteries across multiple renewables sites. 

%\textit{Instead of using techniques that adapt the availability of power to match the computation demand, we can either defer or shift computational demand forward to meet the availability of energy at any instant.} This replaces the concept of a physical battery that stores energy with a \textit{virtual battery} that relies on moving computation temporally.


Viewing energy from this point of view opens a new opportunity. Instead of transferring energy to large data centers and incurring 40-65\% overheads in the distribution and transmission process \shadi{cite}, \seshan{we don't mention distribution/transmission before -- needs to be in previous paragraphy} we are placing an edge data-center (i.e., virtual battery) at the energy production site and dynamically scale computation load to match with energy. 
When energy production reduces, the virtual battery edge decreases power demand by turning off servers all the way down to zero, and when energy production increases, it powers them back on.

\srini{, differentiate with follow the sun. Demand elasticity bi-directional. attribuets of battery, in-situ or substation. DIfferent than leaf node. Taking demand to supply.}
 




% The core concept is to collocate computation alongside renewable energy generation sites (e.g., a mini data-center edge) and dynamically scale computation load to match energy production. 
% When energy production reduces, the edge data-center decreases power demand by turning off servers all the way down to zero (equivalent of "discharging a battery"), and when energy production increases, it can increase power demand by turning on servers (equivalent of "charging a battery"). \shadi{shouldn't it be the reverse?}. This approach is not physically storing electrons, rather it is virtually storing energy by using it ahead of time for useful computation that would have been done in the future. As a result, it can time-shift an infinite number of times. \jinghan{it looks like we are currently offloading local computation to use the energy at neighbor sites.} 


%%%%%%%::: variability shifts to need for availability
% Instead of hiding variability in energy through storage, as done in real batteries, 
This approach introduces a new challenge---\textit{coping with the inherent and frequent unavailability of computational resources}. Applications might loose their assigned resources drastically, unexpectedly, and frequently. 

%%%%%%:: environment & applications targeted
One way to cope with unavailability is by requiring applications to be ``degradable'', i.e., they can quickly adjust to fewer or more resources (high elasticity), and hibernate if no resources are available. This is similar to how applications would run on preemptable resources such as Spot instances and Harvest VMs \cite{harvestvm}\shadi{cite}. 
%However, most current applications do not have such support built in. Also, 
From the infrastructure provider's perspective, preemptable applications are not the most profitable options, e.g., spot instances are \shadi{X\%} cheaper than stable VM on average \shadi{cite}. 
As a result, an economically practical system should maximize the number of applications that the system can improve
availability levels to acceptable levels, and use the spare, variable capacity towards degradable applications.


We observe that \textit{We can boast availability by relying on more than one virtual battery site (multi-VB)}.
Despite the variability in a single renewable site, across different (nearby) locations, times of the day, and with different sources (solar, wind, etc), renewable sources often exhibit uncorrelated and complimentary patterns of energy production (Section ~\ref{sec:availability}). For example, at night-time solar farms have near-zero production while wind resources still have significant production. 

Running applications across multiple virtual battery sites necessitates the use of replication, hot/cold stand-by, and migration, all of which introduce additional network overheads in an often bursty pattern. Based on our results on a 3month solar and wind traces in Europe, migration spikes can be as high as \shadi{X TBs}. \shadi{@Anup: please verify numbers and details}. In addition, this can add latency overheads if sites are placed too far apart.

Multi-VB introduces a new trade-off: for availability applications would want to spread as much possible, however, for networking overhead (and energy consolidation) they would want to be as consolidate as possible. We model this trade-off as a linear optimization problem and show how a proof-of-concept heuristic scheduler can provide significant networking overhead reduction (\shadi{X}\%) while ensuring the availability required by applications. \shadi{@jinghan, please verify and fix, and add numbers.}


% \textit{We can boast availability by relying on more than one virtual battery site}, using replication, a hot/cold stand-by, or migration. However, any of these techniques introduce new network overheads on the WAN in an often spiky pattern. Based on our results on \shadi{vm traces from x}, we see an extra \shadi{x\%} equivalent of more than \shadi{y gbps....}. This can simply overload the limited WAN capacity, often between \shadi{x-y}, creating significant networking bottlenecks. 

% Moreover, all these approaches should be done in an economic manner, considering the dynamic pricing of energy markets, cost of underutilized hardware, etc. 

% In this paper we explore the challenges to realizing the virtual battery concept and propose solutions to these challenges. 


Our main contributions are \shadi{suggestions?}:
\begin{itemize}
    \item Introducing the concept of virtual battery edges that hide renewable variability using a computation shifting paradigm.
    \item Boasting availability of virtual batteries by leveraging multiple virtual battery locations (multi-VB).
    \item Characterizing the network overhead of multi-VB applications and developing a network aware scheduler that places applications across complimentary virtual battery locations.
\end{itemize}

% \srini{Highlight 3 main points - i) in-situ location of VB (lower cost due to transmission loss avoidance), ii) Fat edge, iii) New availability paradigm}.



==> tex/hotnets/intro.tex <==
\section{Introduction}
\label{sec:intro}

% Climate change is the major challenge of our times. To avoid significant repercussions, we need to decarbonize our energy mix sources substantially. 

% Increasingly, governments~\cite{unsdg} and corporations~\cite{pledge} around the world have pledged to become ``carbon neutral'' or ``carbon negative'' in the near-term future. 

%%%%::::: Renewable are the next big thing, but they are variable as well
Cloud computing has become a substantial source of carbon emission, even surpassing the aviation industry~\cite{lean-ict}. As a result, all major cloud providers have pledged to become ``carbon neutral or negative'' in the near-term future~\cite{azurepledge,pledge,googlepledge}. 
Renewable energy sources are an attractive choice for reducing carbon especially since technological advancements have reduced their production costs to values lower than traditional energy sources~\cite{renewablecost}.
However, one challenge in making effective use of renewables
is that their energy production varies significantly over time. For example, solar produces no power at night and daytime power output varies with clouds and across seasons. Similarly, wind production changes frequently based on the direction and speed of wind. 

% {\color{red} Importantly, these variations on energy supply are not always correlated with the energy demand, thus, creating a compounded gap.} \shadi{do we need this sentence? We are not solving this point in the paper.} \anirudh{the flow is breaking here. Can we conclude saying that even combining multiple renewable sources from the same location does not reduce variability to a level that can be tolerated today?}
% \shiv{Importantly, these supply side variations are not correlated with energy demand, so the net imbalance on the grid is compounded by both demand and supply variability.} 

% Specifically, due to this variability, a renewable source may exceed or fall short of the energy needed by a cloud computing system at any moment in time.
% Shiv comment: the problem of variability and matching is not just for cloud computing. It is a matter of matching aggregate supply to aggregate demand when renewables become a larger fraction of aggregate supply and is more volatile (which makes matching much harder) and needs space-time matching & flexibility. 
Existing systems either move energy across space (via transmission lines) or time (using batteries), e.g., using energy from batteries or traditional power generation sources during short-falls, or transmitting to/from the grid during periods of excess/low power generation. However, these solutions have significant shortcomings:  1) traditional non-renewable energy sources have high carbon footprints; 2) transmission lines incur significant overheads ($\approx$ half of the cost is due to transmission and distribution~\cite{fares2017trends})
% (e.g. it costs around 3 cents/kWh for transmission and distribution~\cite{fares2017trends} which translates to $\approx$50\% of the retail cost of electricity) 
and takes decades for installation; and 
3) penetration of grid-scale Li-ion and other chemical batteries are minuscule in scale, e.g., in the US battery capacity is $\approx$ 0.4\% of the overall solar and wind capacity~\cite{storageus,renewableus}.
% and with a limited life-cycle ($\approx 1000-3000$ discharge cycles \shadi{cite}) \anup{implication of limited lifecycle?}.
We need an alternate, more efficient approach to bridge the gap between the properties of renewable energy sources and requirements of cloud computing. 
% , 
% and with a loss of efficiency (\shadi{X\%} loss during charge \& discharge\shadi{cite}). 
% 
% {\color{red}
% To fully bridge the variability gap, we need a \textit{scalable, green, low-overhead option} alongside the current solutions.} \shadi{is this an overclaim? especially the low-overhead part} \anirudh{Something is missing here. We need to say that locations for renewable sources are far away from existing grid? And also that renewable generation tech is far outpacing battery innovations rather than focusing on negatives of Li-ion. The flow is also breaking here. It is not just about fully bridging the variability gap but also about leveraging the full potential of renewables for computing rather than wasting it in losses of transmission and storage.}
% \seshan{AB: I think your points are valid but make the intro a bit too complex. I think these points are better delivered later in the paper/intro.}

% 3) grid-scale Li-Ion batteries which come with  a limited life-cycle ($\approx 1000-3000$ discharge cycles \shadi{cite}), 
% and loss of efficiency (\shadi{X\%} loss during charge \& discharge\shadi{cite}). 
%  \shiv{Given the scale and urgency of the renewables integration challenge, there is room for a variety of options}.\shadi{This sentence seems out of place.}



%%%%%::: introduce problem statement and Virtual battery concept. 
In this work, we propose a paradigm shift:
% \shiv{at the intersection of cloud computing and renewables}:
\textit{Instead of using techniques that adapt the availability of power to match the computation demand, we shift computational demand to meet the availability of power.} We call this \textit{Virtual Battery (VB)} since it relies on shifting computation much like a battery shifts energy across time, and avoids transmission/distribution costs. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{figures/arch.pdf}
    % \vspace{-1.8em}
    \caption{\small The Virtual Battery (VB) based cloud architecture vs the current deployments. %\anup{Can perhaps label the sites, DC and coal factory. Currently a bit hard to make out what the different pieces are.} \srini{pptx file is in figures directory -- also need to add a battery}
    % \anirudh{I think the sizes and number of the DCs should be same on both sides}
    }
    \label{fig:arch}
    % \vspace{-1.5em}
\end{figure}

%replaces the concept of a physical battery that stores energy with a \textit{virtual battery} that relies on moving computation temporally.

As shown in Figure~\ref{fig:arch}, VB design enables a different approach to datacenter deployment. Currently, power is sent from various energy sources through distribution lines to large datacenters, as needed to meet current demand. Power is lost in transmission or battery storage, and non-renewable energy sources are used to meet demand. In the proposed architecture, each renewable energy source is coupled with a datacenter, sized to match local energy production. Computation at each site opportunistically scales up and down to make use of locally generated power. This comes with several economical incentives as discussed in~\S\ref{sec:VB-design}. In practice, we expect a combination of both existing large centralized datacenters complemented by smaller VB edge deployments. 



% Viewing energy from this point of view opens a new opportunity. Instead of transferring energy to large data centers and incurring 40-65\% overheads in the distribution and transmission process \shadi{cite}, 
% %\seshan{we don't mention distribution/transmission before -- needs to be in previous paragraphy} 
% we can place an edge data-center (i.e., virtual battery) at the energy production site and dynamically scale computation load to match with energy. 
% When energy production reduces, the virtual battery edge decreases power demand by turning off servers all the way down to zero, and when energy production increases, it powers them back on.

%\srini{, differentiate with follow the sun. Demand elasticity bi-directional. attribuets of battery, in-situ or substation. DIfferent than leaf node. Taking demand to supply.}
 
% The core concept is to collocate computation alongside renewable energy generation sites (e.g., a mini data-center edge) and dynamically scale computation load to match energy production. 
% When energy production reduces, the edge data-center decreases power demand by turning off servers all the way down to zero (equivalent of "discharging a battery"), and when energy production increases, it can increase power demand by turning on servers (equivalent of "charging a battery"). \shadi{shouldn't it be the reverse?}. This approach is not physically storing electrons, rather it is virtually storing energy by using it ahead of time for useful computation that would have been done in the future. As a result, it can time-shift an infinite number of times. \jinghan{it looks like we are currently offloading local computation to use the energy at neighbor sites.} 


The key challenge associated with the VB approach is that when local power generation dips, servers \emph{must} be shut down. As a result, apps can lose their resources drastically and frequently.
Cloud providers can deal with this resource variation in two ways.
First, 
they can require apps to be ``degradable'', i.e., apps can quickly adjust to fewer or more resources (high elasticity) and hibernate if no resources are available. This is  similar to running on preemptable resources such as Spot instances, and Harvest VMs~\cite{awsspot, azurespot, awsburst,azureburst, harvestvm, sharma2019resource}. Unfortunately, from the cloud provider's perspective, preemptable apps are not the highest value options, e.g., spot instances are 60-90\% cheaper than stable VMs~\cite{spot-prices}. Also, many apps cannot use degradable resources and require high availability.
Thus, we need to maximize the number of resources that assure availability levels similar to the cloud, and only use the spare, variable capacity towards degradable apps.

Second, we observe that \textit{we can reduce resource variability by relying on more than one virtual battery site (multi-VB)}.
Despite the variability in a single renewable site, across different (nearby) locations, times of the day, and sources (solar, wind, etc), renewable sources often exhibit uncorrelated and complementary patterns of energy production and can reduce overall variability by 3.7$\times$ (\S\ref{sec:multi-VB}).
% For example, at night-time solar farms have near-zero production while wind resources still have significant production. 

There are some trade-offs associated with the multi-VB approach. 
Running applications across multiple VB sites necessitates the use of replication, hot/cold stand-by, and migration, all of which introduce additional network overheads in an often bursty pattern. Based on our results on a 3 month solar and wind traces in Europe, migration spikes can be as high as tens of terabytes, which which can consume 40\% of shared WAN capacity (\S\ref{sec:nw-overhead}). In addition, this can add latency overheads if the multi-VB sites are far apart. This factor limits the number of sites in a multi-VB group as networking overhead increases with the number of sites. We model these trade-offs in a linear optimization formulation and show how a proof-of-concept scheduler can provide significant networking overhead reduction.

% To minimize resource variability, applications will want to spread as much possible. However, spreading more widely increases networking overhead. We model this trade-off as a linear optimization problem and show how a proof-of-concept scheduler can provide significant networking overhead reduction, $>$30\% in total reduction in total bytes and \shadi{x$times$} reduction in peak overheads, while ensuring the availability required by applications. \shadi{@jinghan, please verify and fix, and add numbers.} \anirudh{Scale is missing here. 10s of TBs is high or low? Can we say in terms of number of hours of traffic for a representative WAN link?}\shadi{@Anup: can you do a back of envelope conversion to time based on a standard NW link capacity?}

% \textit{We can boast availability by relying on more than one virtual battery site}, using replication, a hot/cold stand-by, or migration. However, any of these techniques introduce new network overheads on the WAN in an often spiky pattern. Based on our results on \shadi{vm traces from x}, we see an extra \shadi{x\%} equivalent of more than \shadi{y gbps....}. This can simply overload the limited WAN capacity, often between \shadi{x-y}, creating significant networking bottlenecks. 

% Moreover, all these approaches should be done in an economic manner, considering the dynamic pricing of energy markets, cost of underutilized hardware, etc. 

% In this paper we explore the challenges to realizing the virtual battery concept and propose solutions to these challenges.
\smallskip\noindent\textbf{Contributions and Roadmap.} Our main contributions are:
\begin{itemize}[noitemsep,nolistsep,topsep=0pt,leftmargin=*]
    \item Introducing the concept of Virtual Battery (VB) cloud edge data centers that absorb renewable energy variability using a computation shifting paradigm (\S\ref{sec:intro}).
    \item Boosting availability of computation scheduled on VBs by leveraging multiple sites (multi-VB) (\S\ref{sec:multi-VB}).
    \item Characterizing the network overhead of multi-VB apps and developing a power \& network aware scheduler placing apps across multiple VB sites (\S\ref{sec:nw-overhead}, \S\ref{sec:solution}).
\end{itemize}

% \srini{Highlight 3 main points - i) in-situ location of VB (lower cost due to transmission loss avoidance), ii) Fat edge, iii) New availability paradigm}.

% \shadi{Maybe add? even to achieve degradable, you have to be smart. consolidation for energy, postponing hibernation for degradable.}


==> tex/hotnets/nw-solution.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{A new networking challenge} 
\label{sec:nw-overhead}

The multi-VB design flattens the variability in energy, however, it introduces a new challenge--\textit{Applications that could regularly run in a single data-center with high levels of availability now \textbf{must} run across multiple sites to achieve similar availability.} Such applications must rely on either hot/cold standbys using continuous replication or migration. This introduces continuous or bursty network overheads on the wide area links connecting sites. Such links may be more constrained given the remote locations of typical renewable energy farms. While replication and migration is a well-known overhead in traditional cloud settings, \textit{the scale is vastly different.} In the cloud, many applications are not geo-replicated. For the ones that are, the migration events are due to failures or load balancing, which are rare and oftenly handled within the same data-center (e.g., zone replication).

\begin{figure}[!t]
    \centering
    \begin{subfigure}[]{0.45\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/nw/Wind_migration_overhead_consolidated_timeseries_1.pdf}
    \vspace{-2em}
    \caption{\textbf{Network overhead over time (1 Week) ---} Out: VM migration out of the site, In: VM migration into the site.}
    \label{fig:nw-overhead}
    \end{subfigure}
    \begin{subfigure}[]{0.45\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/nw/migration_overhead_consolidated_cdf_1-short.pdf}
    \vspace{-2em}
    \caption{\textbf{CDF of network overhead over 3 months of simulation.} CDF 
    only includes non-zero overhead values.
    % CDF is only shown for samples when network overhead was non-zero.
    }
    \label{fig:nw-overhead-cdf}
    \end{subfigure}
    % \vspace{-1em}
    \caption{\small Network overhead of migration in a multi-VB setting with wind power.}
    % \vspace{-1em}
\end{figure}

% \begin{figure}[]
%   \centering
%   \includegraphics[width=\columnwidth]{figures/nw/migration_overhead_consolidated_cdf.pdf}
%   \caption{CDF of migration overhead in GBs for two different policies over 3 month traces of wind and solar power.}
%   \label{fig:nw-overhead-cdf}
% \end{figure}

We performed trace-driven simulations to quantify the networking overhead of multi-VBs as the volume of incoming and outgoing traffic per site due to VM migrations \footnote{As future work, we plan to incorporate migration latency and impact to application's execution time similar to~\cite{akoush2010predicting}.}.
% , and contrast it with typical network load in a traditional data-center setting. Specifically, we study the volume of incoming and outgoing traffic per site due to VM migrations over time.

\smallskip\noindent\textbf{Setup and Workloads.} We instantiate a site with $\approx 700$ servers each with 40 cores and 512 GB memory. We use an Azure production VM arrival trace and Azure's VM allocation policy to assign VMs to servers. We scale the ELIA~\cite{elia} dataset such that the cluster is fully powered at the max power capacity of the farm.
When power decreases, we first power down unallocated cores, then if needed, we migrate out VMs from servers (in a round-robin order). We use an admission control policy that rejects VMs to maintain 70\% utilization (similar to the VM trace). When power increases, we launch previously rejected VMs and consider these as VMs migrated into the site. We use the memory allocated to a VM for estimating migration traffic due to the absence of disk or memory utilization data.

% \shadi{@Anup:remove two policies.}
% We consider two opposing power distribution policies: 1) a consolidation policy that tries to consolidate power to the smallest set of servers, and 2) a proportionally fair policy which tries to fairly spread power to different servers proportional to the number of unallocated cores. When power reduction requires eviction of running VMs, both policies migrate a single VM from servers, taken in a round-robin order until the power budget is met. We use an admission control policy that rejects VMs to maintain 70\% utilization (similar to the VM trace) when the cluster is not fully powered. Later on, when power increases, we launch previously rejected VMs and consider these as VMs migrated into the site. We use the memory allocated to a VM for estimating migration traffic due to the absence of disk or memory utilization data.
% \footnote{In reality, only utilized memory and utilized disk space would contribute to migration. Since we did not have access to actual disk and memory utilization values, we estimate it by assuming the allocated memory is a fair representation of disk+memory utilization.\shadi{I would remove this. it is quite confusing.}}. 



% \smallskip\noindent\textbf{Power Policy.} We assume that the number of cores on a server are proportional to the power routed to the server and use a power policy to decide how power will be distributed to servers. We consider power policies on two extremes: (1) consolidation policy, and (2) proportionally fair policy. The consolidation policy tries to consolidate power to a small set of servers while the fair policy tries to spread power to different servers. Specifically, when power decreases, the fair policy, reduces server power proportional to the number of unused cores, while the consolidation policy iterates through servers and powers down all available cores until the power budget is met. When power reduction requires eviction of running VMs, both policies migrate a single VM from servers taken in a round-robin order until the power budget is met. When power increases, the fair policy starts cores on servers in proportion to the number of powered-off cores, while the consolidation policy iterates through servers and starts all powered-off cores till no more cores can be powered-on. \seshan{is there any difference in the total core count? i.e. in reality I would assume that consolidation could power more cores since there is a fixed baseline cost to powering a server. If there is no difference, perhaps we could cut the comparison part?} \anup{I think so too.}

% \smallskip\noindent\textbf{Conventions.} The VM arrival trace, maintains $\approx 70\%$ utilization when the cluster is fully powered, we use an admission control policy that reject VMs to maintain 70\% utilization when the cluster is not fully powered. Later on, when power increases, we launch previously rejected VMs and consider these as VMs migrated into the site. We use the memory allocated to a VM for estimating migration traffic. In reality, only utilized memory and utilized disk space would contribute to migration traffic. \anup{Talk about typical memory and disk utilizations.}

\smallskip\noindent\textbf{Observations.} 
As shown in Figure~\ref{fig:nw-overhead} (top graph), $> 80\%$ of the power changes don't incur migrations. Since the cluster is running at 70\% utilization, minor variations in power are absorbed by simply powering down un-allocated cores. In the remainder 20\% of the cases, migrations can cause movement of multiple TBs of data which is significant.
For instance, if the migration is to complete within 5 minutes, then a 10 terabyte spike requires $\approx 200$ Gbps network capacity for a single site. This is roughly $40\%$ of the share of WAN capacity per site, assuming $\approx 100$ sites (each with 1000 servers) share an aggregate WAN link with 50 terabits/sec capacity~\cite{b4after}.

% These network spikes would incur a significant overhead on WAN traffic. For instance, say we want VMs to be migrated within 5 minutes, then a 10 terabyte spike requires $\approx 200$ Gbps network capacity for a single site. This is roughly $40\%$ of the share of WAN capacity per site, assuming $\approx 100$ sites (each having 1000 servers) share an aggregate WAN link with 50 terabits/sec capacity~\cite{}. 
% \anup{in 2013 this was 1 Tbps google B4, need citation for now.}

Figure~\ref{fig:nw-overhead-cdf} shows the CDF of migration overhead omitting the zero values. Migration overhead varies significantly with 99th divided by 50th percentile values as high as 18-30$\times$ for in migration and 12.5-16$\times$ for out migration.
In migration, compared to out migration, has smaller spikes but spread further over time, e.g., 7$\times$ smaller 99th percentile for wind.
This is because, minor power reductions are absorbed by under-utilized machines, while minor power gains cause migrations into the site.

% Solar, PropFairPolicy, fraction zero in: 0.84
% Solar, PropFairPolicy, fraction zero out: 0.96
% Solar, PropFairPolicy, in, p0.5: 148.0
% Solar, PropFairPolicy, out, p0.5: 761.5
% Solar, PropFairPolicy, in, p0.99: 2784.35
% Solar, PropFairPolicy, out, p0.99: 9542.869999999974
% Wind, PropFairPolicy, fraction zero in: 0.87
% Wind, PropFairPolicy, fraction zero out: 0.99
% Wind, PropFairPolicy, in, p0.5: 74.0
% Wind, PropFairPolicy, out, p0.5: 1048.0
% Wind, PropFairPolicy, in, p0.99: 2212.829999999999
% Wind, PropFairPolicy, out, p0.99: 16694.794999999795

% wind  in: 99: 2212,  50: 74   ratio: ~30
%      out: 99: 16694, 50: 1048 ratio: ~16
% solar in: 99: 2784,  50: 148  ratio: 18
%      out: 99: 9542,  50: 761  ratio: 12.5


% We observe that when power drops the spike in migration is higher, while when power increases the spike is shorter but spread over time. Respectively for solar and wind, out-migration has a median of 5$\times$ and 14$\times$, and 99th percentile tail of 3$\times$ and 7$\times$ larger than in-migration. Also,  out-migration has a higher percentage of zero values (97\% vs 86\%).
% This is because, minor power reductions are absorbed by increased utilization and there is no need of migrations. Where as, each minor power gains, provides an opportunity to migrate some VM into the site. Thus inward migrations are spread as they occur on every opportunity, while outward migrations are spiky as they occur only when needed.


% When power drops, application have to move, while when it increases, it can also be used by new incoming applications, rather than migrating running ones. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Solving the network bottleneck}
\label{sec:solution}


% \begin{figure}[!ht]
%   \centering
  
%   \begin{subfigure}[]{0.4\textwidth}
%   \centering
%   \includegraphics[width=\columnwidth]{figures/solar_predictions.png}
%   \caption{solar}
%   \end{subfigure}

%   \begin{subfigure}[]{0.4\textwidth}
%   \centering
%   \includegraphics[width=\columnwidth]{figures/wind_predictions.png}
%   \caption{wind}
%   \end{subfigure}
  
%   \caption{Energy prediction of solar and wind in near (recent, day ahead) and far-away future (week ahead). \shadi{@Srini-I:please keep color consistent among two graphs}}
%   \label{fig:energy-prediction}
% \end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth, trim={0 0 0 0.3cm}, clip]{figures/renewable_data_analysis/power_prediction_ts.pdf}
    \vspace{-2em}
    \caption{\small Energy prediction of solar and wind in near (3 hour, day ahead) and far-away future (week ahead). }
    \label{fig:energy-prediction}
    % \vspace{-1em}
\end{figure}

% While running reliable computation in a virtual batteries introduces new networking challenges, it also has its unique characteristic:
Despite networking challenges, VBs have a unique characteristic:
\textit{\textbf{migrations are spiky, but also predictable.}}
% Renewable energy sources have high variability causing big spikes of migration overload (Figure~\ref{fig:nw-overhead}), but at the same time, this variability is often predictable. 
The main source of variability is weather conditions, which can be predicted quite accurately. Figure~\ref{fig:energy-prediction}, shows the power forecasts provided in the ELIA dataset~\cite{elia} (based on weather forecasts). 
As shown, the prediction model is able to predict the near future very accurately, with a mean absolute percentage error (MAPE) for next 3 hour predictions of 8.5-9\% and for day ahead predictions of 18-25\%. Also, for far-away future (week-ahead) the predictions capture the general trend (MAPE of 44\% and 75\% for solar and wind). 
Bulk of migrations occur when there are sharp changes in power (\S\ref{sec:nw-overhead}), which can be predicted with at least a day of notice. Since these are points with sharp drops/increases, they are resilient to small errors in predictions.
% Thus, significant migration points, which generate large loads of data transfer, can be predicted with at least a day of notice. Since these are points with sharp drops/increases in power, they are resilient to small errors in predictions.
This predictable characteristic introduces a complex and yet unique scheduling problem:

\textit{How to schedule applications across highly-variable but predictable capacity locations in a way that i) ensures high level of availability, ii) introduces low \& non-bursty network overheads, and iii) minimizes energy usage?}

There is an inherent trade-off between these goals. To reach higher availability, applications would want to spread their compute across as many uncorrelated and complimentary locations as possible, e.g., different VB sites, racks, and servers. But, this would mean higher network overhead by introducing more migrations and replications and less energy efficiency by powering up more racks, top of rack switches, and servers even though they might be underutilized. 

\begin{figure}[]
    \centering
    \includegraphics[]{figures/vb-solution-overview-arrows.pdf}
    % \vspace{-1em}
    \caption{\small Overview of our scheduling approach %\anup{TODO: add next steps and fix graph} %\shadi{@Anup/Jinghan: can you draw this properly?}
    }
    \label{fig:vb-model}
    % \vspace{-1em}
\end{figure}

For each application, with a number of requested VMs, the scheduler needs to find a group of VB sites that a) are in close proximity to reduce latency overheads of splitting applications, b) have complimentary energy patterns to guarantee availability of resources \& reduce migrations, c) have a good mix of stable and degradable VMs (based on their individual energy patterns) to cope with local power variations.  


To solve this scheduling, we model the cluster of VB sites as a graph (Figure~\ref{fig:vb-model}). Each node represents a VB site and has the energy prediction alongside total and allocated computation capacity. Two nodes are connected via an edge if their latency is below a fixed threshold, $50ms$ in our case. 
We use this model and break the scheduling problem into 4 steps: 1) subgraph identification, 2) subgraph selection, 3) site selection, 4) VM placement. We optimize the placement of incoming applications. As the environment changes, e.g., weather predictions update or applications complete and resources free up, we need to rerun the optimization.


\smallskip\noindent\textbf{1) Subgraph identification.} we identify subgraphs of the VB site graph which have \textit{low latency and complimentary variability}. We formulate this as a k-clique identification and prioritization problem. First, we find all cliques (fully connected sub-graphs) of a given size $k$ ($k$=2 to 5). These are subgraphs with a small latency between any two VB pairs, thus, an application split within such a subgraph would not experience high latency overheads. Then, for each $k$, we sort all subgraphs based on the total coefficient of variability. Identifying dense subgraphs has been a well-studied problem in literature with tractable approximate solutions~\cite{bhaskara2010detecting}.

% \noindent\textbf{2) Subgraph selection:} Subgraph identification can generate large number of subgraphs, e.g., we found \shadi{X} subgraph in the \shadi{Y} dataset. Searching this many subgraph choices quickly becomes prohibitive. Thus, the selection phase filters out a \textit{candidate list of subgraphs} based on future power availability and having a proper mix of degradable and normal VMs that match future energy patterns (similar to Section \shadi{??@anupt the breakdown graph you created}). \shadi{how do we solve this step?} \shadi{should this step really be separate from 3)? }

\smallskip\noindent\textbf{(2, 3) Subgraph and Site selection.} In these two steps we identify the exact site(s) the application should be placed on.
Subgraph identification can quickly generate large number of subgraphs. Thus, first we select a smaller set of subgraphs candidates and for each candidate subgraph find the optimal site placement schedule. For both the steps, candidates/sites are selected to optimize for two things: (1) choosing options that are predicted to maintain good power levels to prevent migrations, 
% (2) ensuring a good mix of degradable and non-degradable VMs in each subgraph/site so power variations can be absorbed by degradable VMs, 
(2) balancing load between subgraphs/sites. We formulate subgraph and site selection as a Mixed-Integer Programs (MIP) with the following two objectives:
\begin{align}
\label{eq:formulation-perf}
\text{O1: Total} &\quad \text{Min} \sum_{i \in apps} migration\_overhead(i), \nonumber\\
\text{O2: Peak} &\quad \text{Min} \max_{i \in apps} migration\_overhead(i), \nonumber 
% \text{O3: Deployment} &\quad \text{Max} \sum_{i \in degradable\_apps}  request\_cores(i) \nonumber
\end{align}

The first order goal is to minimize the total migration overhead (in bytes) while looking ahead in the future. The second order goal reduces the peak migration overhead (in bytes). 
% {\color{red}
% And, the third order goal tries to keep a balance of degradable applications in each location, by maximizing their proportion while satisfying O1 and O2.
% }
Optimizing for O1 and O2 implicitly maintains a balance of degradable applications in each locations allowing handling of abrupt power variations.

% \anup{Having identified good sub-graph(s), we need to decide on which site(s) within the sub-graph(s) should we place the VM(s) on. Subgraph identification can generate large number of subgraphs, e.g., we found \shadi{X} subgraph in the \shadi{Y} dataset. Navigating sites accorss many subgraph choices quickly becomes prohibitive. Hence, we take a two step approach by first filtering out a candidate list of subgraphs and then selecting candidate sites from the candidate subgraphs. For both the steps, candidates are selected to optimize for three things: (1) choosing subgraphs/sites which are predicted to maintain good power levels so that a need to migrate never arises, (2) ensuring a good mix of degradable and non-degradable VMs in each subgraph/site so power variations can be absorbed by degradable VMs, (3) balancing load between subgraphs/sites. To capture these preferences, we formulate subgraph and site selection as a Mixed-Integer Programs (MIPs).}

% \begin{table}[t]
%     \centering
%     \resizebox{0.48\textwidth}{!}{
%     \begin{tabular}{c|c}
%     \hline
%     Constant & Description \\ \hline
%     $N, T$ & Number of clusters, and timestamps \\ 
%     $M, K$ & Number of VMs and Hibernatable VMs \\
%     $c$ & Energy consumption per core \\ 
%     $Cap_{j, t}$ & Energy capacity of cluster $j$ at time $t$ \\
%     $Core_{i}, Mem_{i}$ & VM cores and memory size \\ \hline
%     Variable &  \\ \hline
%     % M & number of VMs \\ \hline
%     % T & total time steps \\ \hline
%     $D_{i,j,t}$ & Placement of VM $i$ on cluster $j$ at time $t$ \\
%     $H_{k,j,t}$ & Placement of Hibernatable VM $k$ on cluster $j$ at time $t$ \\
%     $MI_{t}$ & Migration overhead at time $t$ \\ \hline
%     \end{tabular}
%     }
%     \caption{Constants and Variables}
%     \label{tab:vars}
% \end{table}

% An optimized scheduler should find a good mix of degradable and non-degradable VMs at each cluster and an optimized migration plan by incorporating future energy information.
% We formulate this optimization problem as follows.
% Now consider a muiti-site setting with $N$ clusters, $M$ regular VMs, and $K$ hibernatable VMs. Each cluster has its own energy capacity prediction.
% % For each $VM_i$, let $Mem_i$ and $Core_i$ denote its memory size and the number of cores. If 
% % And let $D_{i,j,t}$ denote the placement of $VM_i$ on cluster $j$ at time $t$. 
% To be aligned with Sec~\ref{sec:nw-overhead}, we quantify the migration overhead as the total memory size of all migrated VMs and we assume the power consumption of each VM is proportional to the number of its cores. The VM deployment should satisfy the power capacity requirement of each cluster. Thus, we have the following objectives and constraints (see Table~\ref{tab:vars} for all the variables).
% % $$ Total(MI) = sum (MI_{t}), \;Peak(MI) = \max (MI_{t}) $$
% % $$ MI_{t} = \sum_{j}^{}  \sum_{i}^{} Mem_i \times max(D_{i,j,t+1} -  D_{i,j,t}, 0) $$
% % alternative representaion
% % $$ Migration \propto \sum{Mem_i} \times Diff_{i,j,t+1}
% % Diff_{i,j,t+1} >= 0
% % Diff_{i,j,t+1} >= D_{i,j,t+1} -  D_{i,j,t}
% % $$

% % \begin{frame}
% % \scalebox{1}{\parbox{.5\linewidth}{%
% \begin{align}
% \label{eq:formulation-perf}
% \text{O1: Total} &\quad \text{Min} \sum_{t \in \mathcal{T}} (MI_t), \nonumber\\
% \text{O2: Peak} &\quad \text{Min} \max_{t \in \mathcal{T}} (MI_t), \nonumber \\
% \text{O3: Deployment} &\quad \text{Max} \sum_{k \in \mathcal{K}, j \in \mathcal{N}, t \in \mathcal{T}} (H_{k,j,t}), \quad \text{\bf s.t.} \\
% \text{C1: Migration}  &\quad MI_{t} = \sum_{i \in \mathcal{M}, j \in \mathcal{N}} Mem_i \times max(\Delta_t~D_{i,j}, 0) \nonumber \\
% &\quad + \sum_{k \in \mathcal{K}, j \in \mathcal{N}}   Mem_k \times max(\Delta_t~H_{k,j}, 0) \nonumber \\
% \text{where, } &\quad \Delta_t~X_{i,j} = X_{i,j,t+1} -  X_{k,j,t} \nonumber \\
% \text{C2: VM}  &\quad \sum_{j \in \mathcal{N}} D_{i,j,t} = 1 \quad  \forall i \in \mathcal{M}, t \in \mathcal{T}  \nonumber \\
% \text{C3: HVM}  &\quad \sum_{j \in \mathcal{N}} H_{k,j,t} \leq 1 \quad  \forall k \in \mathcal{K}, t \in \mathcal{T}, \nonumber \\
% \text{C4: Energy} & \quad \sum_{i \in \mathcal{M}} c*D_{i,j,t} \ \times Core_i \nonumber \\
% &\quad  +\sum_{k \in \mathcal{K}} c*H_{k,j,t}  \times Core_k <= Cap_{j,t} \nonumber \\
% &\quad \forall j \in \mathcal{N}, t \in \mathcal{T}  \nonumber 
% \end{align}
% % }
% % \end{frame}


% \begin{equation}
% \forall i,t \;  \sum_{j}^{} D_{i,j,t} == 1 
% \end{equation}
% \begin{equation}
%   \forall j,t \; \sum_{i}^{} c*(D_{i,j,t} \ \times Core_i + \sum_{k}^{} c*(H_{k,j,t} \ \times Core_k <= Cap_{j,t}
%   \end{equation}
\begin{table}[]
    \centering
    \begin{small}
    %\resizebox{0.48\textwidth}{!}{
        \begin{tabular}{c|cccc}
        \hline
        Policy & Total & 99\%ile & Peak & Std \\ \hline
        Greedy & 306,966  & 7,093 & 16,022 & 1,507 \\ %\hline
        MIP-24h & 236,217  & 3,711 & 80,942 & 4,081 \\ %\hline
        MIP & \textbf{209,961}  & 9,379& 62,753 & 2,697 \\ %\hline
        MIP-peak & 212,247  & \textbf{1,684} & \textbf{1,941} & \textbf{562} \\\hline
        \end{tabular}
        %}
        \end{small}
        % \vspace{-0.5em}
        \caption{\small Comparison of migration overhead (in GBs) between different scheduling policies. }
    \label{tab:mip}
    % \vspace{-2em}
\end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.43\textwidth]{figures/optimization/cdf_all.pdf}
    \vspace{-1em}
    \caption{\small CDF of migration overhead across four different scheduling policies.}
    \label{fig:mip_cdf}
    % \vspace{-1.5em}
\end{figure}

We evaluate our scheduler over a 7 day period with four different policies: (i) \textit{MIP}: that optimizes only the total migration overhead (only O1) but for the entire period, (ii) \textit{MIP-peak}: variant of MIP that optimizes both total overhead (O1) and peak overhead (O2), (iii) \textit{MIP-24h}: a variant of MIP (only O1) that iteratively optimizes total migration for the next day, and (iv) \textit{Greedy}: a baseline greedy policy that always assigns VMs to the site with the most available power;

As shown in Table~\ref{tab:mip}, MIP improves the total overhead by $>30\%$ compared to greedy. Other MIP variations have similar migration overhead (1-12.5\% worse), but significantly better peak overhead. Compared to greedy, MIP-peak shows  $>4.2\times$ improvement at 99th percentile while also being less bursty with a $2.7\times$ lower standard deviation. 
As shown in Figure~\ref{fig:mip_cdf}, MIP-peak achieves this by performing more number of migrations  (74\% zero values vs. 81\% in greedy and 94\% in MIP), but each at a lower volume.


% We conduct two experiment to show that an optimized scheduler can help reduce the migration overhead. Each of them considers a subset of the objectives and constraints in the formulation~\ref{eq:formulation-perf}. The setting of each cluster is similar to Sec~\ref{sec:nw-overhead}, except that four clusters are used in each experiment. In the first experiment, we initialize the placement for all VMs and set them to be non-hibernatable. The problem is solved in two steps -- it first finds an optimal core usage and then finds an optimal placement of VM. (Do we have to mention these implementation details?) We compare the migration overhead among four different policies:
% \begin{itemize}[leftmargin=*,noitemsep,nolistsep]
%     \item \textbf{Greedy}: Baseline greedy policy that always migrates VMs to the cluster with the most available energy;
%     \item \textbf{MIP-step}: MIP-based policy that iteratively optimizes total migration for the next day;
%     \item \textbf{MIP}: MIP-based policy that optimizes the total migration overhead for the entire period (7 days);
%     \item \textbf{MIP-peak}: MIP-based policy that optimizes both total overhead (O1) and peak overhead (O2).
% \end{itemize}
% The results are shown in Table~\ref{tab:mip} and Figure~\ref{fig:mip_cdf}. Greedy policy has the greatest migration overhead in total. But this total overhead can be reduced by $31.6\%$ with MIP policy. While MIP increases the 99-percentile peak overhead, we argue that this can be addressed by a pre-migration mechanism or the MIP-peak policy. }

% In the second experiment, the scheduler optimizes for the mix of workloads. \jinghan{TODO}

\textit{Sources of benefits.} We observe three key insights that allow MIP and its variants to reduce total and peak migration overheads. First, all MIP variants place VMs on sites which are predicted to have stable power in the future. This reduces the need for migrations. Second, MIP variants also maintain a good mix of degradable VMs in line with predicted power availability. Thus, when power reduces, degradable VMs take most of the hit without needing to migrate stable VMs. Lastly, MIP-peak migrates VMs preemptively, spreading out migrations over time and reducing burstiness.

% An orthogonal approach, that can be used with any of the policies,  to further improve the peak migration overhead is \textit{pre-migration of applications}. Given the predictable nature of renewable sources for days ahead, we can run the scheduler ahead of time and use the underutilized network capacity to space out migrations over time.

% This pre-migration could be either a) full-migration: moving the entire application (data and compute), or b) partial-migration: currently moving the data and when the need for migration arises, moving the compute and delta of the new data. In either case, the network overload of migration will spread across a longer interval preventing sharp networking spikes. \seshan{cut this para?} \anup{:(}

\smallskip\noindent\textbf{4) VM placement.} We place VMs onto servers in the assigned VB site to minimize total power usage by consolidating as much as possible. Any state-of-the-art approaches as described in related work can be used for this step. 

% once the VMs are assigned to each virtual battery site, we want to place the VMs such that the total energy usage is minimized, i.e., consolidate as much as possible into fewer machines and racks, while maintaining the SLA levels promised. This problem, is in essence the same as power-aware data-center packing. Any of the state-of-the-art approaches~\cite{protean, borg} can be used for this step. \seshan{perhaps just skip if we don't have much to say}



% As shown in Figure~\ref{fig:energy-prediction}, day-ahead forecasts reasonably predict the actual generation from these renewable sources. Based on these predictions, we can place the VMs among different VB sites to ensure availability. As we discussed earlier, we envision the co-location of VB sites with renewable installations. However, there could be several thousand potential VB sites residing besides renewable installations around the world. 
% Choosing a subset of sites to run a particular VM from such a large set of available sites raises several challenges.   

% % However, we need to address several challenges while choosing the appropriate VB sites. 
% First, the set of VB sites responsible for running a given VM needs to be within a tolerable latency threshold. Thus, proper selection of VB sites is imperative for VMs requiring lower latency, such as interactive workloads, to meet pre-defined latency SLAs. Second, the combined renewable generation from these VB sites must have lower variability. With lower variability, we can reliably run long-running VMs with availability equivalent to a regular VM on hyperscalar data centers. Finally, there could be legal requirements for specific workloads running on servers in a select number of countries, which enforces a geographical constraint on selecting VB sites. Next, we present our approach to select VB sites while mitigating the above challenges.  

% We can think of the network of VB sites as a graph $G(V, E)$ with vertices ($V$) representing individual VB sites and edges ($E$) representing sites connected with latency lower than a pre-defined threshold. To reduce migration and replication overheads, we restrict the migration of a VM among a smaller set of $k$ possible sites. Below, we formulate the selection of VB sites to run all VMs requiring higher availability as \textit{k-Clique Densest Subgraph} problem. 

% \textbf{Problem Formulation:} In our graph G, a \textit{k-clique} is a subset of nodes, $C \subseteq V$, such that $|C| = k$. Also, an edge $e \in E$ connects every two distinct nodes in $C$. Let $\mathcal{C}_{k}(G) \coloneqq$ {$C \subseteq V$ : $C$ is a \textit{k-clique} of $G$} denote the list of \textit{k-cliques} of $G$~\footnote{If $k=2$, $\mathcal{C}_{2}(G) = E$. This is a special case of the above formulation called \textit{k-densest subgraph} problem.}. A subgraph $L$ of $G$ is called a \textit{k-clique} densest subgraph if \textit{L} has the maximum \textit{k-clique} density among all subgraphs of $G$, where the density is defined as $\frac{|\mathcal{C}_{k}(L)|}{|V_{L}|}$.

% This subgraph contains several \textit{k-cliques}. However, running a VM would require the variability of the combined power generation from each of the k nodes (VB sites) in a clique to be minimal. Thus, we then sort the cliques based on the coefficient of variation of the combined generation of each  of the $k$ sites contained in them.    





% There are several other angles to this complex scheduling problem. Below, we discuss some of these research opportunities.  



% \noindent \textbf{Network-aware placement--picking the right mix of applications:} 
% Not all applications create equal amount of migration/replication state. For example, a coin mining application has very limited state, a ML training application a can replicate the training data once and only migrate/replicate the models thereafter, while a database application would require continuous replication or large amount of data with low latency \shadi{better 3rd app?}. Maintaining a balance of applications with large and small amount of state in each location will enable the scheduler to move applications with small amount of state in majority of the cases and move the state-heavy application only when absolutely necessary. However, this should be done in fair way that also maintains the application requirements on availability, e.g., having certain number of replicas at all time. 



% \subsection{Is migration/replication the only choice?}
% Using migration and replication increases availability and hides the effect of sudden power drops. However, not all energy volatilities are sharp changes, necessitating moving the applications. Small, temporary changes can be handled within a single virtual battery site, thus, reducing the network overhead. In this section we discuss a few of such options.

% % \noindent\textbf{Use of a small reliable energy source alongside:} Traditional ways, back-up generators, purchasing from the grid, and using batteries, all come high carbon foot prints. However, using these techniques in small scales, just enough to cope with minor variability, can be a beneficial option economically and environmentally if it can reduce the need for migration/replication.

% \noindent \textbf{Systematic degradation within a virtual battery site:} Another option is to downgrade application resources in a way that the application can still have sufficient progress or quality of service. This can be done by reducing the number of allocated cores, e.g., in Harvest VMs\shadi{cite}, under-clocking the CPUs, hibernating a few of an application's VMs, or consolidating the VMs in fewer nodes or racks in one virtual battery site. 

% \noindent \textbf{A new programming paradigm---carbon-aware, degradable apps:} An alternative option is to rely on applications to degrade their computation requirements without using migration. Degradation is application-specific--only the application knows best \textit{if} and \textit{how much} it can cope with fewer resources. For example, a stream processing app might prefer under-clocked workers but maintaining the same number of VMs/workers (to prevent moving state), while a ML training application might prefer to keep fewer high-capacity trainers (for faster convergence).  

% In addition, as users are becoming more environmentally cautious, the carbon footprint of running their application could become a important factor on if/when to degrade. If running the application when there is insufficient renewable energy comes at the cost of using non-renewable high-carbon resources, the user might decide to pause parts (or all) of the application and resume them in the future. 

% Similar to  ``low power mode'' computation in battery-constrained environments such as mobile computing platforms, we envision a simple carbon-aware API exposed to applications which informs the applications when renewable energy sources are running low alongside the carbon footprint of providing a given energy level at that point of time. Then, applications can decide if/how to degrade. Given the predictable nature of renewable resources, this API could also expose future options, e.g., carbon footprint will decrease by  50\% in the next 15 minute window.


% \shadi{2 extreme, something middle. }

% \shadi{any other options not discussed in this section?}



==> tex/hotnets/relatedwork.tex <==
\section{Related Work}
\label{sec:related-work}
% Other related work not discussed in \S\ref{sec:intro}, can be classified into the following categories:
% \smallskip\noindent\textbf{Variable capacity in the cloud.} 
% Several prior works including Spot VMs, Harvest VMs~\cite{awsspot,azurespot, awsburst,azureburst, harvestvm, sharma2019resource} address variability in demand (not energy) by adaptively reclaiming spare resources. While our goal is to optimize use of stable energy, these approaches can be used to leverage unstable energy within a single VB site. %Our goal is to maximize the stable VMs. Such approaches can be used complimentary to our work to handle minor variations within a single VB site. 
% \anup{Can actually remove this. we already talk about spot/harvest in degradable apps. just add citations there.}

% While we address variability in supply, prior works address similar challenges when addressing variability in demand.
% Several proposals such as Spot VMs~\cite{awsspot,azurespot}, Burstable VMs~\cite{awsburst,azureburst}, Harvest VMs~\cite{harvestvm}, Deflatable VMs~\cite{sharma2019resource} reclaim spare capacity when demand is lower and scale down when the demand for regular VMs is higher. While these constructs allow absorbing minor resource variations within a single virtual battery site, additional techniques are required to accommodate sharp renewable energy variations and frequent drops to zero capacity.

\smallskip\noindent\textbf{Migration, replication and check-pointing.} 
A number of prior works have investigated use of migration~\cite{spotcheck,yank,ruprecht2018vm}, replication~\cite{cully2008remus,lagar2009snowflock} and check-pointing~\cite{scr-checkpoint, dnn-checkpoint} to manage faults and outages. 
A few other prior works~\cite{cidon2015tiered, didona2017okapi, shastri2017hotspot, tributary, spoton, spotcheck, qureshi2009cutting}, have looked at using migration/replication to ensure availability using spot markets. While several of them can be used by our work, the scale of variations in VBs are much higher (e.g., they can go all the way down to zero) such that these techniques don't directly translate to our context. 

% Prior works have also investigated migration, replication, and check-pointing techniques to derive availability and reduce costs using an ensemble of virtual machines from different spot markets or regions~\cite{cidon2015tiered, didona2017okapi, shastri2017hotspot, tributary, spoton, spotcheck, qureshi2009cutting}. Our work pursues similar goals and employs similar techniques but from the provider's point of view and in the context of energy variations. These prior techniques can be employed by users of cloud environments and are complimentary to our work.
% Whereas, \cite{zhang2013survey} looked at cloud interoperability and provided a detailed survey of various approaches for deploying and migrating applications across various geographies and cloud providers. 

% Our work currently considers volume of traffic to measure migration overhead, we plan to extend our work to incorporate migration latency and impact to application similar to~\cite{akoush2010predicting}.

% Migration~\cite{spotcheck,yank,ruprecht2018vm} and replication~\cite{cully2008remus,lagar2009snowflock} are well-studied tools to cope with sudden drops of capacity, e.g., outages in data centers~\cite{liu2011live,ramakrishnan2007live}. All major cloud providers (AWS~\cite{awsav}, Azure~\cite{azureav}, GCP~\cite{gcpav}) offer several availability zones (independent data centers) in the same geographic region. Thus, cloud users can deploy applications for better fault tolerance due to uncorrelated failures while retaining low latency by migrating across these availability zones. There are also approaches mentioned in the literature to use frequent check-pointing to run applications in evictable VMs and uncorrelated VM types~\cite{spotcheck,spoton}. Whereas, \cite{zhang2013survey} looked at cloud interoperability and provided a detailed survey of various approaches for deploying and migrating applications across various geographies and cloud providers. Past works~\cite{cidon2015tiered,didona2017okapi} have also studied geo-replication to make applications run cheaper, faster, and more available. Also, \textit{server hopping}~\cite{shastri2017hotspot} is suggested as an approach to migrate from one spot market to another to reduce the VM leasing cost. At the same time, past works~\cite{chatzipapas2015challenge,akoush2010predicting} have also suggested metrics to identify energy-performance trade-offs and avoid aggressive migration without considering performance overheads. All these techniques are complementary and can be used (or have been used) to improve the virtual battery design further.

%Google live migration at scale~\cite{ruprecht2018vm}

%\shadi{X,Y, Z} have looked at live migrations inter- and intra- data-center and optimizing the down-time. \shadi{They have introduced ....}. %\shadi{X,y,Z} have studied geo-replication and how to minimize the cross data-center traffic. 

\smallskip\noindent\textbf{Power aware scheduling.}
We employ features like frequency scaling, powering down cores/caches/memory units to control power distributed to servers~\cite{david2010rapl, kontorinis2012managing}. For the VM placement,  we rely on a number of prior works~\cite{subramanian2010reducing, wu2014green, oversubscript, david2011memory, von2009power, chatzipapas2015challenge, protean, borg, flex, energyaware, wang2013data}. These minimize energy consumption by considering resource utilization, power consumption, and dynamic voltage \& frequency scaling to perform packing, scheduling, and over-subscription of VMs and workloads within a data center. Energy efficiency can be further improved by tuning workloads~\cite{greenai} and opportunistically turning off unused servers/networking infrastructure~\cite{elastictree, servers-off}.

% Past work has looked at \textit{dynamic voltage and frequency scaling} (DVFS) for power-aware scheduling and in cloud data centers~\cite{von2009power,wu2014green}. DVFS is a widely used approach for memory~\cite{david2011memory} and CPU~\cite{oversubscript} power management. Additionally, for power management in VMs, several works in literature propose reclamation of resources~\cite{sharma2019resource,harvestvm}. Server consolidation~\cite{subramanian2010reducing} is another approach where efficiency in use of power in a data center can be improved by dense packing of VMs. 

\smallskip\noindent\textbf{Energy based elasticity/migration.}
Some works ~\cite{liu2014pricing,bahrami2018data} have looked at adaptively adjusting computation based on the cost of energy (from the grid). Others~\cite{chen2014data,liu2013data} have looked at reducing their peak demand to help stabilize the energy grid. Some approaches~\cite{googleblog} migrate workloads based on energy availability. While these have inspired of our work, they do not address the many challenges of variability for compute or they do not target stable VMs with high availability. 


% \anup{This para mostly talks about pricing and use of batteries/shifting computation and we can probably cite these in intro.} \todo{Specifically, some works have looked at reducing compute during high prices~\cite{liu2014pricing,bahrami2018data} by participating in \textit{demand response} program --- where grid operators incentivize consumers to reduce their energy usage at the time of high energy demand. Whereas reducing peak energy demand that aid in \textit{grid stability} has also been studied~\cite{chen2014data,liu2013data}. We have gained inspiration from such works. However, a key difference in our case is that virtual battery is situation \textit{in-situ} and can absorb volatility from renewables directly, thereby reducing the intermittency of solar and wind resources to affect electricity prices. Further, using virtual batteries at multi-sites with uncorrelated power mix or price profiles makes us different. Moreover, such co-location of virtual batteries with renewables can help reduce electricity costs by avoiding transmission and distribution overheads.}

% Recently works~\cite{googleblog} have also explored use of renewable energy employing techniques such as \textit{follow-the-sun} (or \textit{wind}). However such works only consider elastic/hibernate-able workloads. Our work tries to provide guarantees to a broader class of workloads.

%Several works have looked at varying compute in response to efficient use of data center power~\cite{flex,oversubscript,energyaware}, etc. We directly benefit from such approaches at single virtual battery site to quickly modulate the power usage. Specifically, some works have looked at reducing compute during high prices~\cite{liu2014pricing,bahrami2018data} by participating in \textit{demand response} program --- where grid operators incentivize consumers to reduce their energy usage at the time of high energy demand. Related to the literature in demand response, the idea of temporal and location-aware pricing has been explored~\cite{qureshi2009cutting,wang2013data}. Whereas reducing peak energy demand that aid in \textit{grid stability} has also been studied~\cite{chen2014data,liu2013data}. We have gained inspiration from such works. However, a key difference in our case is that virtual battery is situation \textit{in-situ} and can absorb volatility from renewables directly, thereby reducing the intermittency of solar and wind resources to affect electricity prices. Further, using virtual batteries at multi-sites with uncorrelated power mix or price profiles makes us different. Moreover, such co-location of virtual batteries with renewables can help reduce electricity costs by avoiding transmission and distribution overheads. 

%Recently, Google looked at running workloads during periods with higher renewable mix and lower average carbon emissions from various energy sources~\cite{googleblog}. However, such \textit{follow-the-sun} (or \textit{-wind}) restrict themselves to running only flexible workloads. In our case, we hope to run a much broader class of workloads using renewables and significantly help in the higher proliferation of clean energy in our grid.  





%Cite approaches such as \textit{follow-the-sun} and other demand response approaches. We are different because as we look at running jobs using compute demand and price signals. Further, the use of multi-sites with uncorrelated power mix or price profiles makes us different. 

%Workload modulation~\cite{wang2013data}
%grid load stabilizer~\cite{chen2014data}
%Demand response and pricing~\cite{liu2014pricing,bahrami2018data}
%Peak avoidance~\cite{liu2013data}
%Google follow the sun~\cite{googleblog}
%Cutting energy costs~\cite{qureshi2009cutting}




==> tex/hotnets/todo.tex <==

\section{remaining todos}

\begin{itemize}
    \item 
	\shiv{Another use case of Vb is in placement of these at sub stations that aggregate solar and wind energy supply.}
	\shiv{placement of VB strategic - near renewables, near sub station. Edge DCs. }
	\shiv{New resources co-monetization capability} \shadi{Not sure I understand all the above points.}

    \item \srini{Can have a graph showing CDF of length for which VMs are alive. Also, we can show uncorrelated prices/energy sources from similar geography}\shadi{this would be great, but maybe in later sections, not intro}

    \item \srini{Possibly add price traces showing variations in one zone or multiple zones.}\shadi{how about having this in the economic challenges section?}
	
\end{itemize}


==> tex/hotnets/vbdesign.tex <==
\section{Virtual Battery: System Design}

\begin{figure}[]
  \centering
  \includegraphics[width=1\columnwidth]{figures/VB_Systems.png}
  \caption{Virtual Battery System Design.}
  \label{fig:design}
  \end{figure}

\subsection{Time Series Forecasting}

\subsection{Optimization Engine}


\subsection{Workload scheduling}
There are several ways to modulate power. 

\begin{itemize}
    \item HarvestVM
    \item Frequency Scaling
    \item VM eviction
    \item VM Migration
\end{itemize}

However, these approaches can impact availability. 

List of workloads that can work with lower availability.

\begin{itemize}
    \item Internal workloads
    \item Fault tolerant systems: Hadoop
    \item FaaS
\end{itemize}
